Understanding the Stability of Deep Control Policies for Biped Locomotion

Achieving stability and robustness is the primary goal of biped locomotion control. Recently, deep reinforce learning (DRL) has attracted great attention as a general methodology for constructing biped control policies and demonstrated significant improvements over the previous state-of-the-art. Although deep control policies have advantages over previous controller design approaches, many questions remain unanswered. Are deep control policies as robust as human walking? Does simulated walking use similar strategies as human walking to maintain balance? Does a particular gait pattern similarly affect human and simulated walking? What do deep policies learn to achieve improved gait stability? The goal of this study is to answer these questions by evaluating the push-recovery stability of deep policies compared to human subjects and a previous feedback controller. We also conducted experiments to evaluate the effectiveness of variants of DRL algorithms.

==> arXiv-Stability Analysis of Deep Control Policies for Biped Locomotion/chapters/discussion.tex <==
\section{Discussion}

Biped locomotion control has been a long-standing problem in computer graphics. Tremendous efforts have been put into addressing this problem for decades and the computer graphics community has finally reached to the point where simulated controllers are worth comparing with the performance and capability of humans in terms of robustness, energy-efficiency, agility, diversity, and flexibility. This study would be a stepping stone towards rigorous evaluation of DRL policies for biped locomotion.

Although our experiments demonstrated the push-recovery stability of DRL policies in varied conditions, there are still numerous gait factors, body/environment conditions, types of disturbances, technical issues, and limitations to be addressed in future studies. Currently, the effects of lateral disturbances are evaluated in our study. We can think of many other conditions including disturbances at arbitrary locations and directions, and responses to slipping, tripping, slopes, and uneven terrain~\cite{peng_deeploco:_2017, Wang:2010:SIGGRAPH}. 
%references
%https://dl.acm.org/doi/abs/10.1145/1599470.1599475
%https://dl.acm.org/doi/pdf/10.1145/1778765.1778810

Physiological factors such as effort and fatigue are not considered yet. The dynamics model of our bipeds does not have explicit torque limits. Without torque limits, the biped can withstand arbitrarily strong disturbances with unrealistically fast and strong responses. Fortunately, such an unnatural situation does not occur in our experiments probably because joint torques are implicitly limited in the reference-tracking framework. It is strenuous for human participants to walk in $60^\circ$-crouch. $60^\circ$-crouch walking is less stable than $30^\circ$-crouch walking probably due to fatigue, which is not implemented in our DRL algorithms. The simulated bipeds never get tired in strenuous tasks. Incorporating effort and fatigue into a dynamical system requires the concept of energy/torque minimization, which plays a central role in trajectory optimization algorithms~\cite{al2012trajectory, lee2014locomotion}. However, it is still unclear how the concept can be implemented in the DRL framework. Learning energy-efficient, compliant policies would be an interesting direction for future studies.

In our work, we parameterize the reference motion clip to simulate various walking motions with crouch angles, walking speed, and stride length.
Then the motion is warped according to selected gait parameters and then used to train a control policy.
% 그리고 선택된 gait parameters에 맞게 reference motion을 warping하여 이를 트래킹하게 한다. 
The problem is that, unlike the unwarped reference motion that reflects the dynamics of character, warped motions might not be compatible with the model’s dynamics.
% The unwarped reference motion reflects dynamics of character, while largely warped motions hardly match the dynamics.
However, our gait-conditioned policy can mimic various motions warped by gait parameters. 
This is possible because there is a common control method required to mimic walking motions, and this common control method can be learned through DRL.
The control method can be learned more easily from the motions close to the model's dynamics and serves as a guide for the largely warped motions far from the dynamics.


% 우리는 레퍼런스 모션 클립을 몇 가지 parameter에 대해서 parameterizing 하여 DRL에 사용하였다.
% 변형 되지 않은 레퍼런스 모션 클립은 캐릭터의 dynamics를 반영한다고 할 수 있지만, 레퍼런스 모션 클립이 크게 변형될 수록 캐릭터의 dynamics와 멀어지게 된다.
% 하지만, 우리의 파라메트릭 팔러시는 걸음 파라미터에 의해 와핑되는 다양한 모션들을 흉내낼 수 있다.
% 우리의 파라메트릭 팔러시가 다양한 모션들을 흉내낼 수 있는 이유는, 워킹 모션을 mimic 하기 위해 필요한 공통적인 제어 방식들이 존재하고, 이 공통적인 제어 방식을 DRL을 통해 학습할 수 있기 때문이라고 추정한다.
% 이 공통적인 제어 방식은 캐릭터의 dynamics를 반영하는 걸음걸이로 부터 학습될 수 있고, dynamics와 크게 멀어진 걸음걸이도 학습을 할 수 있게 해주는 가이드 역할을 해준다.

% reviewer 4 said.
% Parametric policies. An interesting and challenging aspect of this study was that reference motion clips were warped to simulate different speeds, step lengths, and crouches. One might assume that such warped clips are not compatible with the model’s dynamics, and whether and how the deep reinforcement learning behaved when trying to learn physically impossible motions, and how this was resolved. This could make for interesting discussion.

% Synthesis vs. reference tracking. It is implied but not explicitly stated that it might be helpful to use very few or no reference motion clips. It might be helpful to raise this as an explicit discussion item, because one of the main advances here is that realistic looking push recoveries are produced based on normal and morphed human walking data. It might also help to discuss the challenges ahead for eventually eliminating reference motion altogether. Or conversely, the possibility of synthesizing new motions based on a particular human individual’s idiosyncratic gait.
% 개인의 고유한 보행

Lessons can be drawn from our experiments for the evaluation and implementation of DRL algorithms. First, gait and stability are strongly correlated. Crouching and stomping gaits that might look unnatural or impaired would be more robust than typical, normal gaits. Therefore, evaluating the robustness and stability of the controller entails gait normalization for a fair comparison. Secondly, including uncertainty and disturbances in the learning phase is imperative for learning robust control policies that mimic human balance strategies. Thirdly, gait-conditioned policies are very useful in terms of computation time and memory usage. The use of adaptive sampling is strongly encouraged to improve the robustness of control policies uniformly across a range of parametric domain.



There are many promising applications we can think of. Interactive graphics applications, such as video games, often show animated controllable characters that hit, react, and fall. Understanding their resilience against disturbances would be useful for better simulation of their interactions. We can also think of an exoskeleton-type walking assist device that generates assist force/torque at the joint of the wearer. Many devices are designed to help the elderly and the handicapped who are exposed to the risk of falls. Walking assist devices equipped with the ability to prevent falls would be highly desirable~\cite{constantinescu2007assistive, low2011robot}. We believe that our analysis in this study will provide a solid basis for designing such devices.
%https://arxiv.org/pdf/1909.10488.pdf





% 2019년 11월 28일 교수님 말씀

% 기존 논문 그림 하나도 못 쓰고, 그래프도 못 쓰고, 데이터만 사용 가능
% drl을 사용한 결과들이 2015년 논문에 나온 패턴들과 비슷하게 아마 나올 거라고 생각하는데, 다르게 나와도 괜찮은 거긴 하고.

% 주의해야 할 점!!
% 우리가 하고 싶은 내용이 먼저 나와야 한다.
% 그리고 이전에 이런 연구가 있었는데 이런 거 사용해서 실험했고, 그랬더니 결과가 이렇게 나오더라 식으로 얘기해야!!

% 우리는 push-recovery 실험을 통해 DRL controller for motions parameterized with crouch angle, walking speed, and stride length 를 두가지 관점에서 분석하였다. 
% 먼저, 사람과 maximal detour distance를 비교하여 DRL controller가 사람과 비교했을 때 더 안정적인지를 비교하였다.
% 그리고 사람의 maximal detour distance에 미치는 요인이 DRL controller의 경우에도 같게 적용되는지 확인하였다.
% 그 결과 DRL controller는 detour distance를 비교하였을 때 사람만큼 push-recovery 실험에서 안정적이었다.
% Maximal detour distance에 미치는 요인도 push timing을 제외한다면 같았는데, 이는 DRL contoller의 경우 push-timing이 maxial detour distance가 아닌 성공률에 영향을 미치는 요인이었기 때문으로 생각된다.
% 두번째로는, 각기다른 training 방법, 예를 들면, w/ and w/o push, brute-force and adaptive sampling이 DRL controller의 push-recovery 성공률에 어떤 영향을 미치는지 살펴보았다.
% 예상대로 training 과정에서 push를 넣은 것이 recovery 성공률을 높이는데에 주요한 영향을 미쳤다.
% 그리고, adaptive sampling이 더 다양한 walking speed, stride length에서 brute-force sampling보다 push-recovery 성공율이 높았다.

% We analyzed the DRL controller for motions parameterized with crouch angle, walking speed, and stride length through two push-recovery experiments.
% First, we compared the maximum detour distance with humans to see if the DRL controller is more stable than humans, and also confirmed that the factors affecting the maximum detour distance of humans are equally applied to the DRL controller.
% As a result, the DRL controller was as stable in the push-recovery experiments as humans in the detour distances comparison.
% The factors affecting the maximal detour distance for DRL controller were also the same for human except for the push timing, because the push-timing decides the success or failure, not the maximal detour distance.
% Second, we examined how different training methods, such as with and with out push, brute-force and adaptive sampling, influence the success rate of push-recovery of the DRL controller.
% As expected, the push in the training process had a major effect on increasing the recovery success rate, and the adaptive sampling showed higher push-recovery success rate than brute-force sampling at various walking speeds and stride lengths.

% % 발을 딛는 위치는 biped controller가 안정적으로 걷기 위해 중요한 요소임이 잘 알려져 있으나, 이에 대한 정량적인 분석은 부족했다.
% % 우리는 이전 사람 실험 데이터에서 사람이 밀렸을 때 발을 디디는 위치를 stance foot 기준으로 계산하여, external push가 있을 때 어떻게 달라지는지 확인하였다.
% % 그리고 DRL controller를 push와 함께 트레이닝한 경우 push 없이 트레이닝 한 경우에 비해 진행방향 쪽으로 발을 덜 내딛게 됨을 확인하였다.
% % 이는 사람 실험 데이터에서 확인한 부분과 일치한다.
% It is well known that the foot stepping is an important factor for the biped controller to walk stably, but the quantitative analysis was insufficient.
% In the human experiment data, we calculated the position of the foot stepping when the person was pushed, based on the stance foot, to see how it changed when there was an external push.
% In addition, when the DRL controller was trained with push, it was confirmed that the foot stepping location was less toward the direction of progress than when training without push.
% This is consistent with the findings in human experimental data.

% % 이 실험의 한계점은 다음과 같은 것들이 있다.
% % 각 관절이 낼 수 있는 토크에 제한이 없어서, 필요한 경우 캐릭터는 unrealistic 한 힘을 낼 수 있는 가능성이 있다. 하지만 proportional and derivative gain 로 제한된 PD control을 쓰기 때문에 그런 경우가 생길 가능성은 적다.
% % 이 실험에서는 왼발이 stance foot임을 가정하고 왼쪽에서만 밀었다. stance foot과 다른 방향에서 external force가 가해지는 경우 (예를 들면, 왼발이 stance foot이고 오른쪽에서 미는 경우) 전혀 다른 foot placement strategy가 필요할 것이다. 이번 실험에서 Deep RL이 사람과 비슷한 foot placement strategy를 학습한다는 것을 알았기 때문에, 반대방향에 대해서도 사람과 비슷한 strategy를 보이는지 확인하는 것도 좋은 미래 연구가 될 것이다.
% % 이 실험에서 캐릭터는 self collision이 없는데, 사람이 3 번의 발걸음으로 recover 하는 경우 다리가 꼬이는 것을 막기 위해 self collision을 염두에 두고 움직일 가능성이 있으며, 이는 maximal detour distance의 값에 영향을 미쳤을 것이다.

% The limitations of this experiment are as follows.
% There is no limit to the torques of joints can produce, so the character has the potential to produce unrealistic torques. However, this is unlikely because the joint torques are calculated from PD control which limited to PD gains and differences between target and current joint angles.
% In this experiment, the character is pushed only on the left side with assuming the stance foot is the left foot. If an external force is applied in a different direction than the stance foot (for example, the left foot is a stance foot and a character is pushed from the right), a completely different foot placement strategy will be required. Since this experiment shows that DRL controller learns a foot placement strategy that is similar to humans, it would be a good future study to check that the foot stepping strategy of the human and a DRL controller are similar when the push direction is opposite.
% In this experiment, the character has no self-collision. If a person recovers in 3 steps, it is possible to move with keeping self-collision in mind to avoid twisting the leg, which may have affected the value of the maximal detour distance.


% To explore the possibility and the limit of the DRL as a tool for producing the biped controller, we first trained several controllers using DRL by changing the conditions, conducted push-recovery experiments, gathered simulation data, and analyzed the data. 



% Our goal is to answer the questions in the introduction. 
% drl로 학습한 컨트롤러가 사람의 stability에 대적할만 한가?
% 이 질문에 답하기 위해 우리는 사람의 데이터와 이전 시뮬레이션 데이터와의 비교를, 여러가지 지표를 통하여 알아보았다. 그리고 결과적으로 그렇다고 할 수 있다.
% 우선 detour distance를 보면, normal gait보다 crouch가 덜 밀려서 더 안정적으로 나오는 경향성도 같고, 심지어 수치도 비슷한 레벨로 나왔다. 또한 통계분석을 해봤을 때에도 역시 이전 논문에서 찾아낸 gait factors들이 다 유의미하다고 나왔다. 다음으로 cot도 사람과 같이 파라볼릭한 형태로 나왔다. foot placement를 비교해봤을 때, 사람과 시뮬레이션 결과가 상당히 흡사하게 나왔다.

% 그렇다면 drl controller가 사람의 밸런싱과 비슷한 정책을 사용하는가?

% 이 질문에 답하기 위해 우리는 세 가지 variation을 정하고 각각의 combination으로 여덟 가지 controller를 training하였다. drl controller 간의 비교는 실험 성공률을 사용했다.

% push를 넣고 학습한 것과 그렇지 않은 controller를 비교해봤을 때, 당연히 push training의 성공률이 훨씬 높았다. 외부 힘이 가해졌을 때 foot placement 정책이 중요하다고 알려져 있다. 따라서 미는 힘의 크기가 커질 수록 밀린 방향으로 발을 더 멀리 디뎌서 중심을 유지할 거라고 예상했는데, no push training controller 의 경우는 예상과 같은 결과였으나, push training의 결과는 달랐다. 미는 힘과 미는 방향 축으로의 발 위치가 비례하는 것이 아니라, 어느 순간부터 곡선형태가 나왔다. 그리고 시뮬레이션 모션들을 분석 결과 힘이 커지면 foot placement strategy를 one step recovery에서 three step recovery로 바꾼다는 것을 관찰하였다. 즉, 너무 큰 힘으로 밀리면 one step 만에 균형을 잡을 수 없다는 것을 학습하고 step을 더 사용하여 균형을 잡는 정책을 학습한 것이다. 
% 외부 섭동을 넣고 보행을 학습했더니 사람과 같이 힘의 크기에 따라서 유연한 foot placement strategy를 학습했다는 점이 큰 의미가 있다. 

% 컨트롤러의 표현력과 자유도를 위하여, we did parameterization for the walking speed and step length. 그러나 이로 인하여 안정성은 떨어질 수 있다. 파라미터라이제이션없이 한 개의 레퍼런스 모션만을 학습한 컨트롤러에 대해 실험했을 때 성공률이 더 높을 것이다. (실험해볼 수 있을 듯.)
% 하나의 crouch level, 또는 모든 crouch level에 대해서 학습한 컨트롤러의 비교도 이와 일맥상통하다고 생각한다. 
% 외부 섭동을 트레이닝했느냐 안 했느냐가 중요한 factor였다. 외부섭동을 트레이닝했을 시에는 하나의 모션만 학습한 컨트롤러의 실험 성공률이 더 높아서 더 안정적이라고 할 수 있다. 그러나 외부섭동 없이 트레이닝한 컨트롤러의 경우는, 오히려 여러 개의 다양한 모션을 학습하기 때문에, 더 컨트롤 범위가 넓어지는지 normal gait와 crouch 20도의 경우에는 실험 성공률이 더 높았다. trade-off???? 

% parameterization을 하면서 parameter sampling을 어떻게 하느냐도 안정성에 영향을 줄 수 있다. uniform과 adaptive sampling 두 가지를 사용해서 training을 해 보았고, 결과적으로 adaptive sampling의 실험 성공률이 uniform sampling 성공률보다 높게 나왔다. 여기서 디스커션할 거리가 뭐지?????

 
% 본 연구를 통해 DRL을 사용한 biped controller가 외부 섭동에 대하여 사람과 비슷한 밸런싱 정책을 하고 있다는 것을 알 수 있었다. DRL이 사람의 밸런싱 정책을 학습할 수 있다는 것에서, 시뮬레이션을 사용하여 사람의 움직임에 대한 비밀들을 탐구해볼 수 있는 가능성을 볼 수 있다.
% 사람의 보행 제어기가 겉보기에만 사람과 같은 게 아니라 내부 매커니즘 적으로도 실제 사람과 가까워 지고 있다는 점이 괄목할 만하다. 앞으로 그래픽스 뿐만 아니라 재활이나, 의학 분야, exoskeleton 분야에서 시뮬레이션을 활용할 수 있는 가능성이 높아질 것 같다. Quantitative measure를 통하여 시뮬레이션 간의 비교도 가능하고, 사람 데이터와의 비교도 가능하다. 

% \begin{itemize}
%   \item DRL controller가 사람보다 더 잘 걷는가?
%   \item DRL controller가 외부힘을 사람보다 더 잘 버티는가? - 외부힘을 잘 버티도록 training한 controller를 사람보다 잘 버틴다고 말 하는 것이 의미가 있는가? 
  
%   A. detour distance 면에서는 사람과 비슷한 정도로 버틴다. ( joint torque 모델 - push training - each crouch - uniform)
% 성공률은 50\% 정도. 성공률 면에서는 외부힘을 사람만큼 버틴다고 할 수 없다.
%   \item DRL controller가 사람과 비슷한 strategy로 외부 힘을 버티는가? - main이 되는 질문.
%   \item DRL controller와 사람이 외부힘을 버티는 strategy를 무엇으로 어떻게 비교할 것인가?
%   \item DRL controller가 사람과 비슷한 strategy로 버티기 위해서는 어떻게 학습을 해야 하는가? 
  
%   A. ( joint torque 모델 - push training - each crouch - uniform) is best at this moment.
% 왜 이게 제일 좋은가?
%   \item DRL controller의 캐릭터 모델이 사람과 비슷할수록 비슷한 strategy로 버티는가? 
%   \item DRL controller가 외부힘을 더 잘 버티기 위해서는 (성공률을 높이기 위해서는) 어떻게 학습을 해야 하는가? 
  
%   A. 큰 힘으로 트레이닝을 한다. 타이밍에 대해서는?
%   \item DRL controller가 외부힘을 더 잘 버티기 위해서는 캐릭터 모델이 어떻게 구성되어야 하는가? 
  
%   A. DRL controller with pushed, normal walking motion vs. with unpushed, pushed walking motion 
%   \item 이전 controller와 비교 가능한가?
%   \item 실제 사람이 디디는 발의 위치와 DRL controller가 디디는 발의 위치는 (특히 실패한 경우에) 어떠한 차이가 있는가?
%   \item 실패한 데이터로부터 배울 점이 있는가?
%   \item 학습하는 캐릭터의 모델이 달라지는 것은 학습에 어떠한 영향을 미치는가?
%   \item DRL controller를 학습하는 도중에 밀고 밀지 않고의 차이가 어떤가?
%   \item 학습하는 방식의 차이(uniform, adaptive)는 학습에 어떠한 영향을 미치는가?
%   \item 성공률이라는 새로운 measure 제시
% \end{itemize}


% There are pros and cons when using DRL controller. 
% % DRL controller를 사용했을 때의 장점과 단점 
% %장점
% 특별한 human insight를 사용하지 않고 사람의 모션데이터를 바탕으로 하여 컨트롤러를 학습하였기 때문에, 사람이 걷는 동작을 따라하도록 reward function을 디자인함으로써, balancing과 gait하는 원리를 implicit하게 얻어낼 수 있었다. drl controller로 시뮬레이션한 모션들이 보여주듯이, 외부섭동이 일어났을 때 반응하는 모습이 자연스럽고 사람과 비슷한 양상을 보인다.
% %단점...
% Overfitting issue.
% 사람의 모션 데이터를 인풋으로 받기 때문에, 다른 morphology의 character에는 적용하기 어렵다. (retargeting issue) 
% 또 학습 모션 데이터 이외의 다른 모션들은 시뮬레이션 불가능하다. 

% 실제 push 실험한 사람 모션 캡처 데이터를 tracking하도록 한 컨트롤러와 normal walking에 push한 것을 학습한 컨트롤러 비교하면 의미가 있나?
% 실제 push 실험한 사람 모션 캡처 데이터를 tracking 하도록 학습하는 것에 대해 얘기했었는데, 그 데이터들이 다 제각각 skeleton scale이 다르기 때문에 그걸 맞추지 않고 그냥 joint angle 따라가라라고 하면 DRL이 어느 정도 학습할 지를 모르겠어.

% ys: parameter 뽑는 방법에 대해서 discuss할 수 있다.
% 생각을 해보니 normal distribution으로 파라미터 뽑으면, 평균에서 멀어질 수록 (즉 일반적인 보행 동작에서 멀어질 수록) 동작의 난이도(?)는 어려워지는 반면 더 적은 학습 기회를 가지게 되는 셈이라서, 왠지 맞는 방법이 아닌 것 같아.
% 어쩌면 정담이 올해 논문처럼 각 parameter별 marginal value function을 이용해서 adaptive sampling을 해야하는 건 아닌가 싶기도 하고.
% 일단은 normal distribution과 uniform sampling 두 가지 방법으로 학습시켜서 학습 진행 상황을 비교해보면, 정말 adaptive sampling이 꼭 도입해야 하는 critical한 부분인가를 판단할 수 있지 않을까?
% 만일 adaptive sampling을 한다면 에피소드 중간에 push를 넣는 여부에 대해서도 고민을 해야할 것 같은 것이,
% 정상보행보다 crouch 60이 안정성이 떨어져서 더 밀리는데, adaptive sampling을 하면 그런 경우도 억지로(?) 안정적이 되도록 사람보다 훨씬 효과적인 정책을 학습할 수 있지 않을까 싶기도 하고..
% push 없이 학습하는 정책이 사람의 보행을 최대한 잘 흉내낸 정책일까? 그럴 수도 있고, 아닐 수도 있고..
% 어쩌면 push 없이 학습하면 push를 좀 가하면 말도 안 되게 쉽게 넘어질 수도 있고 (reference state에서 확 벗어나기 때문에 사실 이럴 가능성이 제법 클 듯)
% 여하간 이 모든 것들이 실험을 해보면 사람-시뮬레이션 비교 분석 뿐만 아니라 시뮬레이션-시뮬레이션 간의 학습 방식에 따른 차이를 discussion하기 좋은 부분들이라, 논문의 내용을 풍부하게 만드는데 도움이 될 꺼리들인 것 같아.




==> arXiv-Stability Analysis of Deep Control Policies for Biped Locomotion/chapters/introduction.tex <==
\section{Introduction}

The simulation and control of human locomotion is a central issue in physically-based animation. The design principles of biped controllers have pursued several fundamental goals: Simulated locomotion should look human-like, should be resilient against unexpected disturbances, and should be interactively controllable to change its walking direction and speed. It is also desirable for the controller to be able to generate various gait patterns and transitions. We are particularly interested in the second goal and understanding the balance recovering capability of biped controllers. 

Many design approaches have been explored to construct robust biped controllers: feedback control laws~\cite{conf/siggraph/HodginsWBO95, yin2007simbicon}, data-driven control (in the sense that the controller mimics a reference motion)~\cite{sok2007simulating, lee2010data, 2016-TOG-controlGraphs}, nonlinear/stochastic optimization~\cite{Lasa:2010:SIGGRAPH, Wang:2010:SIGGRAPH, kwon_momentum-mapped_2017}, model-based optimization~\cite{Coros:2010:GBW:1778765.1781156, Mordatch:2010:SIGGRAPH, tsai2009real}, and reinforcement learning~\cite{2018-TOG-deepMimic, yu2018learning}. In particular, recent advances in deep reinforcement learning (DRL) have made significant improvements in the simulation and control of biped locomotion. There are many variants of DRL algorithms for learning locomotion control. A typical example-guided algorithm takes a short motion clip as input and learns a control policy (a.k.a. controller) that allows the biped to imitate the dynamic behaviors captured in the motion data~\cite{2018-TOG-deepMimic}. Alternatively, DRL algorithms can produce control policies conditioned by continuous, user-controllable gait parameters, which may include walking speeds, steering angles, body shape variations (e.g., leg/arm lengths), and a large repertoire of action choices captured in unorganized motion data sets~\cite{Won:2019, bergamin2019drecon, Park:2019}.  

Although deep control policies are substantially more robust than the previous state-of-the-art, many questions remain unanswered. Are deep control policies as robust as the balance-recovering capability of human locomotion? Do simulated locomotion use similar strategies as human locomotion to maintain balance? Does a particular gait pattern similarly affect human and simulated locomotion? Are conditioned control policies as robust as unconditioned control policies without adjustable parameters? What do deep policies learn to achieve robustness in locomotion? 

% \color{red} 
% In this paper, we proposed 
% % To answer to these questions, we train the several kind of deep control policy 
% Before answering these questions, we train deep control policies able to cover the various gait conditions (e.g., walking speed, stride length, the level of crouch, push timing, and push force), which we call them as "gait covering policies".
% Fisrt, we train deep control policies able to cover the various gait conditions (e.g., walking speed, stride length, the level of crouch, push timing, and push force). Second, we conducted push-recovery experiments to evalutate the stability of deep control policies. 
% 걷는 도중 외부힘이 적용되었을 때 어떤 요인이 영향을 미치는지를 탐구하고, 사람의 데이터와 biped controller의 stablity를 비교하는 Research 가 진행되었다~\cite{lee2015push}. 우리는 이 연구와 동일한 세팅을 하기 위하여 파라메트릭 팔러시를 학습하였고, 동일한 실험 환경을 조성하여 push-recovery test를 진행하였다. 그리고 나서 quantified measure를 사용하여 stability를 비교하였다.  
% \color{black}

In this paper, we evaluate the push-recovery stability of deep policies under various conditions (e.g., walking speed, stride length, the level of crouch, push timing, and push force). To do so, we conducted simulation-based stability tests with each control policy we trained and compared its stability with previous human/simulation experiments. The push-recovery stability measures how well the simulated biped withstands impulsive pushes. More specifically, two measures are adopted in our experiments: maximum detour distance and fall-over rate. 
%We measured how the biped detours in the direction of modest pushes and how often it falls over at the presence of larger pushes. 
The detour distance measures how far the biped detours in the direction of modest pushes to assess the resilience of human walking without falling over. The fall-over rate is more popular for assessing the stability of simulated controllers because the experiments can be conducted safely in the simulation environment with a wider range of push magnitudes. The characteristics of control policies are analyzed qualitatively and quantitatively based on post-push foot placement patterns. 

We also evaluate the effectiveness of DRL variants. Gait-conditioned policies have many advantages over unconditioned, gait-specific policies in terms of computational time and memory usage. It has been believed that those advantages are gained at the cost of sacrificing the balance capabilities to some extent. In our experiments, we observed that gait-conditioned policies are not necessarily inferior to gait-specific policies in terms of push-recovery stability. It has been also found that adaptive sampling in the gait parameter domain results in more robust policies than na{\"i}ve non-adaptive learning, and learning with random pushes results in more robust policies than learning without random pushes. Random disturbances in the learning process not only improve resilience but also allow DRL policies to better emulate human balance strategies in the foot placement analysis. Overall, we found that DRL policies are as robust as human walking.

%\color{red} 
% The contributions of our paper include

%The contribution of our paper is that we analyze the control poliices trained using DRL to understand the push-recovery stability.
% To the best of our knowledge, this is the first study to quantitatively analyize the gait stability of a simulated biped controlled by DRL. 
%We conducted push-recovery experiments and compared the gait stability between a human and controllers and between controllers based on two stability criteria (detour distance and success rate). Through our study, we suggested what should be considered when training the human movement with DRL for achieving stability.
% 우리의 지식으로, 이 연구는 DRL을 사용하여 제어하는 simulated biped의 안정성을 실제 사람의 안정성과 정량적으로 비교한 최초의 연구이다.
% 우리는 다양한 속도 및 보폭을 가지는 걸음걸이에 대해 두 가지의 안정성 기준을 바탕으로 사람과 컨트롤러, 그리고 컨트롤러 간의 안정성을 비교하였다.
% 또한, 연구 결과를 통해 DRL로 캐릭터의 움직임을 학습할 때 어떤 것을 고려해야 하는지 를 제언하였다.
%\color{black}

% % \subsection{New version}

% Human locomotion is the fruit of responses of moving complex neuro-musculoskeletal body systematically, after sensing the environment around and processing it at the brain. Therefore, it is challenging to find out what factors affect human walking. 
% %Interestingly, the deep learning mechanism resembles that of humans.
% % deep learning mechanism 은 사람의 그것과 닮았다.
% %Deep learning 은 주어진 task를 위해, 수만개의 시그모이드 펑션들이 얽혀있는 여러 layer들로 이루어진 복잡한 구조를 가지고 있는 네트워크의 파라미터들를 학습한다. 정확히 파라미터들이 어떤 의미인지 알지 못해도 그 것들이 만들어낸 네트워크가 task를 잘 만족시키면 장땡인 것이다. 사람의 움직임도 신경, 근육, 관절이 복잡하게 유기적으로 움직여서 수많은 동작들을 해내는데, 이런 사람의 움직임을 표현하는 데 Deep learning이 딱일지도 모른다.
% % 그래픽스 연구자들은 수 십년간 사람의 동작을 재현하려는 시도의 연구들을 계속 해왔고, 최근에는 Deep reinforcement learning (DRL) 을 사용한 캐릭터 제어에 성공하였다 \cite{2018-TOG-deepMimic, lee2019scalable}. DRL은 주어진 state가 있을 때, 어떤 action을 취하느냐에 따라 reward를 받고, 이 reward를 maximum으로 받는 네트워크를 내놓는 학습 방식이다. 목표하는 바 (goal)를 성공시키기 위해 시행착오 (trial-and-error)를 거치며 학습한다는 idea는 사람이 어떤 동작을 깨우칠 때와 흡사하다. 
% Graphics researchers have been doing research for decades to attempt to reproduce human behavior. Recently, they succeeded to control the character using deep reinforcement learning (DRL) \cite{2018-TOG-deepMimic, lee2019scalable}.
% DRL is a learning method that trains a network to get a maximum reward by doing an action when a state is given. The idea of learning through trial-and-error to achieve a goal is similar to when human learns a certain movement.
% % A robot-like humanoid having motor-joint actuated by joint torque or a musculoskeletal model which actuates joints using the force generated by adjacent Musculotendon units similar as the way real human does can succeed to simulate from walking to very complicated skills like cart-wheel or backspin.
% % real human system과 같이 Musculotendon으로부터 힘을 발생시켜 관절을 actuation하는 까지 걷는 것부터 cart-wheel이나 backspin과 같은 어려운 동작들도 문제없이 재현하는 데 성공하였다. 

% 그러나 (기존의 컨트롤러보다) DRL 컨트롤러가 과연 사람과 비슷한 퍼포먼스를 낼 수 있는지, 비슷한 식으로 동작을 배우는지에 대해서는 알려진 바가 없다. 우리는 사람의 가장 기본적인 walking이라는 동작으로 한정하여 이 walking이라는 동작을 배울 때 DRL 컨트롤러가 과연 어떤 아웃풋을 낼 수 있는지를 탐구해보려고 한다. 
% Biped walking simulation 에서 stability (balancing)과 자연스러움 (사람의 동작과 유사한지)가 중요하다.
% 보행안정성에 관련한 연구 중에서, 사람과 시뮬레이션에 대하여 push recovery 실험을 하여 밀린 거리 (detour distance)라는 measure로 안정성을 비교한 연구결과가 있다 \cite{lee2015push}. 우리는 이 실험결과의 human 데이터와 measure를 사용하여, 우리가 디자인한 DRL 컨트롤러와 비교하려고 한다. 
% % 사람의 자연스러운 움직임을 재현하기 위해서 data-driven control을 많이 사용한다.

% % 컨트롤러 디자인을 위해서는 다음과 같은 고려사항들이 있다.
% % 사람과 유사한 밸런싱 정책을 배우기 위해서는 어떤 컨트롤러 디자인이 필요할까?
% % 어떤 캐릭터 모델이 더 사람과 같이 자연스러울까?
% % stability, 밸런싱, 넘어지지 않고 안정적으로 걷는 보행 제어기를 위해서는 어떤 컨트롤러 디자인이 좋을까?
% % 과연 사람의 메커니즘과 비슷한 musculoskeletal model과 DRL 방법이 좋은가?


% 우리의 DRL 컨트롤러 디자인을 위해 four variations (The number of motion data, motion parameter sampling method, presence of push force, and character model) 를 고려했다. 
% 먼저 학습할 reference data가 여러 개일 때와 한 개만을 사용했을 때, 어떤 컨트롤러가 외부 힘에 더 강건한가를 생각해 볼 수 있다.
% 사람은 어떤 동작을 학습할 때, 그 동작만 연습하지 다른 여러가지 동작을 한 번에 학습하지 않는다. 따라서 우리는 후자의 경우가 더 사람과 비슷한 학습 방식이라고 유추해볼 수 있다.
% 다음으로, 보폭과 걷는 속도, 웅크린 정도에 대해서 paramiterization을 하고, 사람의 distribution 데이터에 근거하여 sampling한 parameter들에 대해서 에디팅된 walking motion을 따라가도록 디자인된 컨트롤러에서 sampling method가 결과에 영향을 미칠 수 있다.
% 우리가 사용한 사람 데이터에서의 파라미터들 (walking speed, stride length)은 모두 normal distribution을 그리는데, 그러면 평균 위주의 모션 파라미터들을 뽑으면 학습이 잘 될 것이고, 엄청 느리거나 빠른 걸음,  혹은 보폭이 매우 작거나 크거나 한 unusual한 걸음이라면 학습이 잘 안 될 것이다. 만약 이런 어려운 걸음들까지 커버하도록 하려면 학습이 안 되는 모션들을 더 많이 sampling하도록 장려해줘야 한다. 이는 adaptive sampling을 사용하여 해낼 수 있다.   
% 우리는 uniform sampling과 adaptive sampling을 사용하여 학습된 컨트롤러들을 비교해보려고 한다. 사람의 경우 어떤 스포츠를 배워서 성공시키려고 할 때, 안 되는 동작 위주로 더 해보며 연습한다. Adaptive sampling이 더 사람과 비슷한 방법이므로 보행안정성면에서 더 우월한 결과를 예상할 수 있다.
% push recovery 실험은 사람이 걸어갈 때 옆에서 밀어보는 실험이다. 사람은 자신이 걸어갈 때 외부 힘이 가해진다는 것을 예상하는 경우와 예상하지 못하는 경우가 있다. 우리는 학습 시에 push force를 apply한 경우와 하지 않은 경우를 나눠서 두 가지 컨트롤러를 학습해보았다. 당연히 예상하건대 push force를 학습한 컨트롤러가 더 보행안정성이 높을 것이다. 
% 마지막으로, 과연 joint torque 모델을 사용했을 때와 musculoskeletal model을 사용했을 때 어떤 것이 외부힘에 더 안정적인가를 비교해볼 수 있다. 사람과 더 비슷한 모델은 musculoskeletal model인데 이 모델이 joint torque model보다 더 안정적일지, 또는 사람처럼 외부힘에 반응할지 두 가지 컨트롤러를 비교해보려고 한다. 

% % 모든 동작 한 번에 학습 vs. 한 번에 한 동작만 학습
% % Uniform sampling vs. adaptive sampling
% % push 에 학습된 상황 vs. no push 
% % musculoskeletal model vs. joint torque model
% % \color{red} 각각의 의미 부여하기 \color{black}

% 보행 안정성 측정 및 데이터 결과 분석을 위해서는 어떤 measure가 필요하다.
% 사람데이터와 DRL 컨트롤러 데이터 결과 비교에서는 이전 논문에서처럼 detour distance measure를 사용하였고, DRL controller간의 비교에서는 success rate of push recovery experiment 를 사용하였다. \color{red} 또한 foot placement를 비교해보았다. \color{black}


% 우리는 이에 대한 답을 찾기 위하여, 최신의 data-driven DRL biped control framework \cite{lee2019scalable} 를 사용해서 각 컨트롤러를 학습시켰다. 그리고 push-recovery 실험을 진행하여 결과를 분석해보았고, 다음과 같은 결론을 도출할 수 있었다.

% \color{red}
% DRL 컨트롤러는 detour distance measure로 비교해봤을 때, 사람과 비슷하게 안정성을 갖고 보행을 재현할 수 있다.
% 아래와 같이, 한 모션을 파라미터는 adaptive sampling으로, 외부힘을 줘서 근골격 모델을 사용하여 학습된 Controller가 안정성이 가장 높았다. 이는 사람이 어떤 동작을 학습할 때 하는 방식과 유사하다는 점에서 의미가 있다.
% \color{black}

% \begin{itemize}
%     \item Training for one motion  >  Training for several motions
%         % 한 번에 한 동작만 학습 > 여러 동작 한 번에 학습 
%     \item \color{red} Adaptive parameter sampling > Uniform parameter sampling \color{black}
%     \item Training with external push > Training without push
%          % push 에 학습된 상황    >   no push 
%     \item \color{red} Musculoskeletal model  >  Joint torque model \color{black}
% \end{itemize}

% \subsection{Old version}

% % hp: 딥러닝하고, 사람의 기본적인 워킹 얘기하고 엮으면 될 것 같긴 한데, 고민되는 것이.. 이미 push recovery paper 가 있는데 이 논문과 겹치는 부분이 많은데 많이 겹쳐도 괜찮을까요?
% % ys: 이전 논문 애기 간략하게 하고, 여기서 보여줄 새로운 거에 대한 얘기가 더 많이 들어가야, 딥 러닝과..
% % 예전에는 이런 한계가 있었고(제한적인 feedback rule에 따라서, 단순한 밸런싱을 하는 밸런싱 정책을 따랐기 때문에)
% % 실제 사람의 behavior를 반영하는지는 클리어하지 않다. DRL은 액션을 학습하는 거기 때문에 차이가 있다. 더 표현력이 좋다?

% % Previous researches about biped controllers

% % 그래픽스에서는 사람의 움직임을 자연스럽게 모사하려는 연구들이 계속 진행되어 왔다.
% Biped walking is a major topic in many research areas such as robotics, biomechanics and computer graphics. 
% % 로보틱스, 그래픽스, 바이오메케닉스 등 여러 분야에서 사람의 기본적인 움직임인 워킹에 대해 연구하고 있다. 
% % Especially in computer graphics society, there have been many hard works for simulating human locomotion.
% Thanks to the many studies, a few principles or insights of biped walking were known.
% For example, human tends to walk at the speed where consuming metabolic energy expenditure minimally \cite{ralston1976energetics}.
% Symmetry can yield robust movement without falling \cite{patterson2008gait}. Stepping at the right location is an important thing for balancing.
% By using these prior knowledge came from physics and biomechanics, animation researchers have been working on simulating human walking.
% In consequence, many controllers were designed for decades, and they showed reasonable results.
% % 이러저러한 방법들로 controller design 하는 연구들이 진행되어 왔는데, 넘어지지 않고 이족보행하는 결과들을 보여주었다.

% % 그동안 그래픽스 분야에서 사람의 워킹을 시뮬레이션하기 위해서 연구들을 많이 해왔다.
% % Gait simulation에서 중요한 factor가 두 가지가 있다고 했다. 자연스러운가, balancing 잘 하는가.
% % 넘어지지 않고 걷기 위해서는 balancing이 중요한데, 이를 위해서 phase별로 나눠서 feedback control하는 방법들을 사용하였다 \cite{yin2007simbicon}. 
% % For achieving the naturalness of human movement, data-driven control is used \cite{lee2010data}.
% % 사람 움직임의 자연스러움을 얻기 위해서 data-driven simulation 방법들이 도입되었다 \cite{lee2010data}. 또는 최적화를 통하여 controller를 만드는 연구들도 있었다. 

% However, there is a limit to express human-like stable motion in many respects. 
% In reality, human locomotion is the fruit of responses of moving complex neuromusculoskeletal body systematically, after sensing the environment around and processing it at the brain. Therefore, it is challenging to find out what factors affect human walking.
% % 어떤 factor들이 얼마만큼의 가중치로 영향력을 미치는가를 정확하게 알아내는 것 자체가 어려운 것이다. 
% % 실제로 사람의 움직임은 주변 상황들을 센싱하여 이를 뇌에서 처리하고, 복잡한 신경근골결모델들을 유기적으로 움직이면서 반응한 결정체인데, 이를 단순한 캐릭터 모델과 단순한 컨트롤 방법으로 모사하였기 때문이다.
% % Limitation of the previous study
% % However, 기존 연구들은 단편적인 기준들만을 사용하여 이를 optimization에 적용하는 등 한계점이 있었다.
% Previous controllers are designed manually just relying on human insight, so balancing strategies followed simple and restricted feedback rule for balancing. Also, these controllers are made suitable for the specific motion, morphology or environment, therefore, they cannot deal with different motions/character models and handle the unexpected situation. In short, the generalization is one challenging problem for producing the controller.
% % 또한 특정 동작에 맞춤형으로 컨트롤러를 만들기 때문에 리타케팅이라던가 여러가지 동작에 적용가능한 범용 컨트롤러는 제작이 어려웠다. 또한 어떤 예상치 못한 상황이 왔을 때 ( ex, 누가 밀었다던가), 이에 대해 적절하게 반응하는 컨트롤러를 만들어내는 것은 더 어려운 문제였다.
% % 이 것이 stability이고 이 것이 사람다운 움직임인 것이다. 기존의 컨트롤러들은 이런 것까지 캐치해내지 못했다. 이런 변화에 대응할 수 있는 능력까지 컨트롤러가 담아낼 수 있는 여지가 있는 것인가? 
% Meanwhile, previous researches used simplified character model compared human body, such as the character model in 2D with lower body, inverted pendulum model or the full body model that uses the joint torque actuator. 
% % And the foot model is simplified having one or two segments that hinder the foot's functionality.
% % 지나치게 단순화된 full body 모델을 사용하여 2D, 하체만, 아니면 inverted pendulum 같은 모델, 토크 모델만 사용한다던가, 박스 foot을 사용한다던가 이런식으로 character model이 너무 단순하였다.
% Using the simple control method and character model is not sufficient for representing realistic human gait.
% For human-like character movement in movie or game industries, for exoskeleton research in the robotics society, and for the diagnosis and comparison of pre- and post-operation in the field of medicine and rehabilitation, there is a need to use computer simulation. Thus, exquisite character modeling and controller design are required for more human-like and precise biped simulation.
% % 애니메이션 게임 산업에서 자연스러운 캐릭터의 움직임을 위해서, robotics society에서 exoskeleton 연구, 의학이나 재활 분야에서도 진단이나 수술전후 경과비교를 위해서 컴퓨터 시뮬레이션을 사용하려는 움직임이 있다. 따라서, 더 자연스럽고 더 정밀한 수준의 biped simulation을 위해서는 업그레이드된 캐릭터 모델링과 컨트롤러가 필요하게 되었다.

% % researches about biped controllers using Deep reinforcement learning  
% Recently, there are researches using deep reinforcement learning (DRL) for designing biped controllers \cite{2018-TOG-deepMimic, lee2019scalable}. In these work, DRL can learn the balancing strategy of real human implicitly from the motion capture data. They proved the robustness of their controller by showing the marvelous results including many human locomotion from the basic walking to acrobatic movements such as backflip and cartwheel. 
% % DRL로 만든 컨트롤러를 사용해서 여러가지 모션들이 잘 시뮬레이션되고 있다. 
% Human can learn the new motor skills fast, and has outstanding adaptability for the change of the environment. DRL learns from trial-and-error as human does, therefore we believe that using DRL for making a controller is quite promising way for simulating human motions. 
% % 사람은 새로 배우는 동작들을 잘 학습하고, 외부 환경 변화에 적절히 대응하는 능력이 있다. DRL의 학습하는 방식이 사람이 학습하는 방식과 유사하므로, drl 컨트롤러로 나온 모션들이 사람의 움직임과 꽤 근접한 결과들을 보여주었다 promising results.

% % Our goal (challenge)
% However, it is not easy to answer the question of how good the performance of the controller learned using DRL is. 
% % There are many things to survey: training 과정에서 뭘 뺄 것인가 넣을 것인가...
% We want to know the ability of DRL biped controller compared with human, or the existing feedback controller.

% % 그러나 DRL을 사용하여 학습된 컨트롤러의 성능이 과연 어느정도인가라는 질문에 대답하는 것은 쉽지 않다. qualitative or quantitative analysis 방법이 아직 부족하기 때문이다. 
% % 또한, Human biped walking을 위한 여러 개의 컨트롤러들이 고안되었지만, 상대적으로 컨트롤러 디자인에 대한 고찰이나 컨트롤러들의 성능 비교, 대조를 위한 연구들은 많이 진행되지 않았다. 
% % 우리가 하고 싶은 것은 DRL 컨트롤러가 어느 정도로 사람 보행 패턴, 그리고 stability를 잘 학습하는지에 대한 답을 하고 싶다. 또한 기존의 컨트롤러보다 더 stable한지 비교해 볼 수도 있을 것이다. 

% % push recovery stability research 
% There is existing research that can help to answer these questions. Lee et al \cite{lee2015push} conducted push-recovery test for evaluating the stability of the biped controller. In this work, they used existing feedback controller \cite{lee2010data} to extract the simulated walking data and analyzed simulated results compared with human data. As a result of the analysis statistically using Bonferroni test, they identified four decisive factors (crouch, gait speed, timing and magnitude of push). It can be very helpful in designing controllers in the aspect that it can extract significant factors. Moreover, it is meaningful in a way that it can measure the stability of the controller quantitatively by using the travel distance after the push-recovery test. 
% % 이러한 질문에 도움을 줄 수 있는 기존 연구가 있었다. Lee et al \cite{lee2015push}은 컨트롤러의 stability를 measure하기 위해 push recovery test를 진행하였다. 이 연구에서는 기존의 feedback controller \cite{lee2010data}를 사용하여 모션 데이터를 추출한 후, 사람의 데이터와 비교하였다. Bonferroni test를 사용하여 통계적으로 데이터들을 분석한 결과, 여러가지 factor 후보군 중에서 네 가지 decisive factors (crouch, gait speed, timing and magnitude of push)를 발견해내었다. 이 연구는 유의미한 factor들을 선별할 수 있다는 점에서 컨트롤러 디자인에 도움이 많이 될 수 있다. 또한 push-recovery 실험을 통해 얻어낸 recovery distance로 quantitatively 컨트롤러의 stability를 measure할 수 있다는 면에서 큰 의미가 있다. 

% % how to set up
% We train the DRL controller, conduct experiments under the same experimental setting of Lee et al \cite{lee2015push}, extract simulated data, and analyze the results statistically.
% In addition, to investigate the difference in walking stability as the model changed, two full body character models actuated with muscle or joint torque were used.
% % , and a simple foot and a multi-segment foot model were used.
% % 우리는 이 연구에서 사용한 실험 세팅과 동일하게 환경을 조성하고, controller를 drl을 사용하여 트레이닝하였다. 또한, joint torque full-body model 외에도, musculoskeletal model, 좀 더 진화된 발 모델 등 캐릭터 모델을 바꿔보면서 실험하여보고, 보행 안정성에 어떤 유의미한 차이를 주는지도 알아보고자 하였다. 실험 결과 데이터를 뽑은 후, 통계적으로 기존 데이터들과 비교 분석을 실시하였다.

% % experiment results

% \begin{itemize}
%     \item Training each crouch motion separately is more robust than when training all crouch motions.
%     \item Training with push force is more robust than training without push force. 
%     \item \color{red} Foot placement is important.??
%     \item Training using adaptive sampling than using uniform sampling of parameters shows more robust robust results with push force. 
%     \item Which character model we use affects the stability..?? \color{black}
% \end{itemize}


==> arXiv-Stability Analysis of Deep Control Policies for Biped Locomotion/chapters/method.tex <==
\section{Biped Locomotion Simulation}

% Figure
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/model_skel.pdf}
    \caption{Our full-body dynamics model. Green balls and blue cylinders represent ball-and-socket (3 DoF) joints and revolute (1 DoF) joints, respectively.}
    \label{fig:model}
\end{figure}

Our full-body biped model has rigid bones connected by 8 revolute joints (elbows, knees, and toes) and 14 ball-and-socket joints. The total degrees of freedom (DoFs) of the model is 56 with unactuated 6-DoFs root joint. The biped is 1.7 meters tall and weighs 72 kg. The articulated skeleton is physically simulated and actuated by joint torques (see Figure~\ref{fig:model}).

In this study, we consider two versions of DRL-based algorithms for stability analysis: gait-specific and gait-conditioned. The gait-specific algorithm serves as a common component of recent biped simulation studies \cite{2018-TOG-deepMimic,lee2019scalable}. It takes a short reference motion clip as input and learns a control policy using reinforcement learning. This example-guided control policy represented by a deep neural network provides a distribution of plausible actions at every state. A series of plausible actions sampled from the distributions would drive the biped to track the reference motion while maintaining its balance.

The gait-conditioned algorithm exploits a family of reference motion clips parameterized by user-controlled parameters, such as walking speed and stride length. The gait-conditioned control policy learns how to deal with variations in gaits and styles. Learning a gait-conditioned policy is more computation-efficient and memory-efficient than learning a grid of gait-specific policies in the parametric domain, since each individual gait-specific policy should be learned from scratch. %We will examine if these efficiencies are achieved by sacrificing the capability of the control policy.



\subsection{Gait-specific Policies}

The state of the biped $s=[p,\dot p,\phi]$ includes the positions and velocities of the body links relative to the body coordinate system attached to the skeletal root. $\phi\in[0,1]$ is a normalized phase that matches the temporal span of the reference motion. The output of the control policy is a PD (Proportional Derivative) target that generates joint torques through PD control. The reward function is
\begin{equation}
    r = ( {w}_{q}{r}_{q} + {w}_{v}{r}_{v} ){r}_{e} + {w}_{g}{r}_{g},    
\end{equation}
where ${r}_{q}$, ${r}_{v}$, and ${r}_{e}$ are the reward for tracking reference poses, joint velocities, and positions of end-effectors, respectively. The end-effector and position/velocity tracking rewards are multiplied as suggested by Lee et al.~\shortcite{lee2019scalable}, since they are reinforcing each other. ${r}_{g}$ encourages the biped to walk along a straight line and thus come back to the line after an external push. We set ${w}_{q} = 0.8$, ${w}_{v} = 0.1$, and ${w}_{g} = 0.1$.
\begin{equation}
\begin{split}
    r_q &= \exp \left( -\frac{\lVert \hat{\mathbf{q}} - \mathbf{q} \rVert ^2}{\sigma_{q}} \right) \\
    r_v &= \exp \left( -\frac{\lVert \hat{\dot{\mathbf{q}}} - \dot{\mathbf{q}} \rVert ^2}{\sigma_{v}} \right) \\
    r_e &= \exp \left( -\frac{\lVert \hat{\mathbf{p}}_{e} - \mathbf{p}_{e} \rVert ^2}{\sigma_{e}} \right) \\
    r_g &= \exp \left( -\frac{\lVert \mathrm{dist}(\mathbf{d}, \mathbf{p}_{c}) \rVert ^2}{\sigma_{g}} \right).
\end{split}
\end{equation}
Here, $\mathbf{q}$ is an aggregated joint angle vector, $\dot{\mathbf{q}}$ is a time derivative of $\mathbf{q}$, and $\mathbf{p}_{e}$ is an aggregated vector of end-effector positions.
The hat symbol indicates values from the reference motion.  $\mathrm{dist}(\mathbf{d}, \mathbf{p}_{c})$ is the distance from the center of mass (CoM) of the character $\mathbf{p}_{c}$ to the straight line $\mathbf{d}$.

We used Proximal Policy Optimization \cite{schulman2017proximal} and generalized advantage estimation \cite{schulman2015high} to learn a policy function that maximizes the expected cumulative reward. The learning process is episodic. Many experience tuples are collected stochastically from episodic simulations. In each episode, experience tuples are generated by sampling actions from the policy at every time step and the policy is updated systematically by a batch of experience tuples. We refer the readers to the work of Peng et al.~\shortcite{2018-TOG-deepMimic} for implementation details.

Even if the control policy is learned with a reference motion clip, the exploration strategy of reinforcement learning examines unseen states around the reference trajectory to achieve a certain level of resilience to withstand small unexpected disturbances. The control policy can be even more robust if it learns how to cope with disturbances and uncertainty in the learning process. It has been reported that randomly pushing the biped in the episodic simulations would result in improved robustness \cite{Wang:2010:SIGGRAPH, Park:2019}.
In each episode, we applied random force for 0.2 seconds to push the biped sideways from left or right. The detailed values of push magnitude and timing used in the learning process will be described in section 5.
% The magnitude of the pushes was in the range of 100N to 300N. 

% push training할 때 어떤 식으로 했는지 기술.
% XXX~To make robust controller for external forces, a character is pushed in DRL training.
% A push magnitude and push timing on gait cycle in DRL training are decided using sampling from each distribution of human data.
% We apply only one push at 8-th step, and push direction (left, right) is randomly selected for symmetry.

% External force에 대하여 robust한 controller를 training하기 위해 학습 중간에 캐릭터를 push해준다.
% 이 때 push의 magnitude와 timing은 normal distribution of human data에서 sampling하여 적용하였다.
% Timing은 네 번째 걸음에 swing할 때 밀어준다.
% direction 은 왼쪽 오른쪽 random하게 밀어주었다.


\subsection{Gait-conditioned Policies}

\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{figures/crouch_level.pdf}
    \caption{Crouch gaits. The knee angles of normal, $20^{\circ}$, $30^{\circ}$, $60^{\circ}$ crouching at the middle of the right foot stance phase. }
    \label{fig:crouch_level}
\end{figure}


Human locomotion can be characterized by a family of parameters. The flexibility and representation power of deep neural networks allow parametric variations in gaits to be learned in a single network-based policy, which takes those parameters as state input. The state of the gait-conditioned policy $s=[p,\dot p,\phi,c,l,v]$ includes three gait parameters $c,l,v$, which are normalized crouch angle, stride length, and walking speed, respectively. The stance knee is supposed to be straight at the middle of the stance phase in normal gait. The crouch gait has its knee flexed throughout the stance phase (see Figure~\ref{fig:crouch_level}). The crouch angle indicates the level of crouching normalized to $[0,1]$. The stride length and walking speed are normalized to have zero mean and one standard deviation. 

Because a gait-conditioned policy should deal with gait parameters as state input, learning a gait-conditioned policy requires a collection of example motions that span a target parametric domain. We generate example motions by kinematically varying a single reference motion clip, which represents a normal gait with average walking speed and stride length. Given parameter values $(c, l, v)$, the use of hierarchical displacement mapping and time warping edits the reference motion clip to have the desired stride length $l$, crouch angle $c$, and walking speed $v$~\cite{lee1999hierarchical}.

During episodic learning, the initial state of each episode is taken from the state space containing the target parametric domain. A common way to determine the initial state is to sample uniformly in the state space. This na{\"i}ve learning of a policy often suffers from a biased exploration problem. Many DRL algorithms tend to explore successful regions in the target domain more aggressively while leaving less successful regions unexplored in starvation. For example, human walking is more stable when it crouches to lower down its CoM~\cite{Schafer87}. The control policy parameterized by a crouch angle would explore crouch walking more frequently than normal (straight-knee-at-stance) walking. Consequently, the learned normal gait in the policy would be less robust.

Recently, Won et al.~\shortcite{Won:2019} proposed an adaptive sampling method to deal with parametric body shape variations. We adopt their sampling idea to learn our gait-conditioned policies. The key idea is to give more opportunities to less successful regions in the target domain. The measure of success is a marginal value function $V_m(s_\alpha)$ that estimates the sum of expected rewards for each gait parameter $s_\alpha=(c,l,v)$.
\begin{equation}
    V_m (s_{\alpha})= \int_{{S}_{\beta}} V(s_{\alpha}, s_{\beta}) p_{s}(s_{\alpha}, s_{\beta}) d s_{\beta},
\end{equation}
where $V(s)=V(s_\alpha,s_\beta)$ is a value function which approximately measures the cumulative reward when the controller follows current policy from state $s$, $s_{\beta}$ is a state vector excluding gait parameters, $S_{\beta}$ is the domain of $s_{\beta}$, and $p_{s}$ is a density function which is assumed a constant. The probability of exploring $P ({s}_{\alpha})$ is 
\begin{equation}
    P ({s}_{\alpha}) = \frac{1}{Z}\exp \left( -k \left( \frac{V_{m} ({s}_{\alpha}) }{\mu} - 1\right) \right).
\end{equation}
Here, $\mu$ is the expectation of $V_m$, which is updated along with $V_m$, $Z$ is a scaling factor to normalize $P$, and $k$ is the value that decides the degree of uniformity of $P$ over gait parameter space. MCMC (Markov Chain Monte Carlo) sampling with the probability aims to make the marginal value function $V_m(s_\alpha)$ near-uniform across the domain of $s_\alpha$. We chose $k = 1$ for all controllers.
% except for $60^{\circ}$-crouch walking whose $k = 0.5$. We sacrificed uniformity for better learning since $60^{\circ}$-crouch walking is challenging to learn. 


%For each crouch angle, the stride length $l$ and the walking speed $v$ are sampled from a joint distribution based on the human experiment data~\cite{lee2015push}. Specifically, we calculate the mean and the covariance matrix of $l$ and $v$ for each crouch angle, and get a 95\% confidence region with assumption that $l$ and $v$ follow multivariate normal distribution in human data. Once the confidence region is determined for each crouch angle, two kinds of sampling method are used to sample parameter values ($c$, $l$, $v$); uniform sampling and adaptive sampling. Sampled gait parameter values ($c$, $l$, $v$) then decide one edited motion clip, and the motion clip becomes an input of an episode.

%Among the gait parameter values, there are values suitable for a character to walk stable, and values that are relatively difficult to walk because the crouch angle can be large, walking speed can be slow or fast, or the step length can be large or small. Uniform sampling draws these values with equal probability. Since the gait parameter values that are easy to walk are learned faster than the values that are not, the experience tuples for the easy to walk are collected as the training proceeds more than the difficult. Because of this, uniform sampling may not be able to learn over all parameter values in the sampling region.

% Recently, Won et al.~\shortcite{Won:2019} proposed adaptive sampling method for various character shapes and control variables.
% The main idea is to give more opportunity to the difficult when training.
% More specifically, adaptive sampling encourages the experience tuples for the difficult to control are to be collected more than uniform sampling does.
% In our application, a gait parameter value that is expected to have a smaller sum of rewards has a higher probability of sampling.
% To estimate a sum of the reward for each gait parameter ${s}_{\alpha} = (c, l, v)$ which is included in the state vector, we use a marginal value function $V_m ({s}_{\alpha})$~\cite{Won:2019} which evaluates an expected value for gait parameter, and update the function in the learning process.
% \begin{equation}
%     V_m (s_{\alpha})= \int_{{S}_{\beta}} V(s_{\alpha}, s_{\beta}) p(s_{\alpha}, s_{\beta}) d s_{\beta}
% \end{equation}
% where $V(s)$ is a value function which approximately measures the cumulative reward when the controller follows current policy from state $s$, $s_{\beta}$ is a state vector except state of gait parameter $s_{\alpha}$, and $S_{\beta}$ is a domain of $s_{\beta}$.
% Based on the marginal value function, an adaptive sampling probability function $P ({s}_{\alpha})$ for each gait parameter values is available:
% \begin{equation}
%     P ({s}_{\alpha}) = \frac{1}{Z}\exp \left( -k \left( \frac{V_{m} ({s}_{\alpha}) }{\mu} - 1\right) \right).
% \end{equation}
% Here, $\mu$ is the average of $V_m$, which is updated along with $V_m$, $Z$ is a scaling factor to normalize $P$, and $k$ is the value that decides the degree of uniformity of $P$ over gait parameter space. We chose $k = 1$ for all controllers except crouch $60\,^{\circ}$ whose $k = 0.5$ is used, because it is more tough to learn than other crouch levels.


% % Figure
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/models.pdf}
%     \caption{Full body character model: joint torque model (left), and musculoskeletal model (right).
% % (c) simple foot model, (d) multi-segment foot model. 
% }
%     \label{fig:model}
% \end{figure}

% We used two types of full-body character models: a skeleton model and a musculoskeletal model (Fig.~\ref{fig:model}).
% Each model is 1.7 meters in height and weighs 72kg.
% Bones are modeled with the rigid bodies which are articulated with 8 revolute joints (elbows, knees, thumbs and the other toes) and 14 ball joints.
% Musculoskeletal model consists of 284 line muscles attached to the bones.
% A skeleton model is actuated joint torques, while Hill-type line muscles are used to move a musculoskeletal model.
% Also, we use two kinds of foot models. Simple foot model consists of three segments having two toes and a sole, while the multi-segment foot model has 12 revolute joints with 31 muscles.



% \subsection{DRL Training for Biped Controller}
% % \subsection{DRL Training}
% % For the data of DRL controller, 

% \color{red}
% We used the state-of-the-art DRL controller for a musculoskeletal character \cite{lee2019scalable}. 
% Previous feedback controller has to use optimization-based for parameterization. 
% 그러나 DRL은 컨트롤 factor들을 파라미터라이제이션해서 학습 가능하다는 파워풀한 장점이 있다.
% 따라서 여러가지 실험 설계가 가능하다.
% 예를 들어 사람은 push recovery 실험을 할 때, body com을 낮춰서 (몸을 낮춰서) 안정성을 높이려고 한다.
% crouch 정도를 자유롭게 선택할 수 있도록 열어주고 외부힘을 가하면서 controller를 학습했을 때 과연 사람과 같은 식으로 최적화가 될 것인가를 실험해 볼 수 있다.
% \color{black}
% % 예전 feedback controller들은 0도와 60도 모션만 가지고도 다른 각도들을 시뮬레이션 하는게 가능했다. 그러나 drl에서는 학습데이터에 포함되지 않은 정보들은 (crouch 각도나 stride length, walking speed) 재현이 불가능하였다. \color{red} 좀더 파지티브하게 설명해야 하나...? 어쨌든....이유설명 필요! \color{black}
% % 먼저 사람데이터와 비교할 시뮬레이션 데이터를 얻기 위해, 우리는 사람데이터의 모션을 tracking하면서 external push에 강건한 controller를 각각 training하였다. 
% In the previous study, they used five parameters (level of crouch, walking speed, stride length, push force and push timing) for the experiments, and we used same parameters for training the DRL controller.
% % 이전 논문에서 human experiment data을 가지고 사람의 보행 안정성에 영향을 미칠 수 있는 possible factors 31가지의 combination으로 Linear Mixed Model (LMM) 여러 개를 테스트해본 결과, AIC BIC를 가장 최소화하는 FACTOR 조합을 찾았는데, crouch, walking speed, stride length, push force and push timing 이다 \cite{lee2015push}. 우리는 이 factor들을 DRL에서 컨트롤 파라미터로 사용하여 학습할 것이다. 
% We use one normal gait motion for training, modify input reference motion as respect to parameters at the start of the each episode.
% Then DRL learns a policy to imitate the modified motion.
% Note that the walking speed and the stride length have strong correlation so we sample parameters considering the co-variance of the two to avoid an extraordinary pair of parameters.
% % (정확하게는 parameter들이 이루는 multivariate gaussian distribution에서 중심부터 ellipsoidal 한 형태로 확률을 accumulation 하는 cumulative distribution function을 생각했을 때, 95\% 확률을 가지는 parameter set 안에서 uniform 하게 뽑고 있어요. 각 parameter에 대해서 uniform하게 뽑으면 step length는 큰데 walking speed는 작다거나 하는 extraordinary한 parameter가 나올 수 있어서요.)


% % We train a controller for each level of crouch motion. We use one normal gait and create the crouch reference motions (crouch $20\,^{\circ}$, crouch $30\,^{\circ}$, and crouch $60\,^{\circ}$) by using the hierarchical motion displacement mapping \cite{lee1999hierarchical}. Note that level of crouch is the only discrete parameter of the previous study.
% % 레퍼런스 모션마다 컨트롤러 각각 학습시켰다.
% % discrete parameter인 crouch angle (0, 20, 30, 60)이 있어서, 모션 네 개를 나눠서 학습하도록 하였다. 
% % Each motion, we modify the given reference motion as respect to the stride length and walking speed at the start of the each episode and DRL learns to imitate the modified motion. We use uniform sampling for parameterization for the robust training for all kinds of motions. Note that we consider the covariance of parameters when sampling.

% % 그래서 drl 트레이닝 할때는 매번 episode마다 (crouch angle, step length, walking speed)를 사람 모션 캡처에서 얻은 normal distribution에 따라 뽑아서 학습하려고 했는데, 아무래도 학습하는데 시간이 오래 걸리는 것 같네요.ㅎㅎ 학습을 한창 돌리고 있긴 한데 좀더 지켜봐야할 것 같아요.

% We define the state s = [$p$, $\dot{p}$, $\phi$, $c$, $l$, $v$], where $p$, $\dot{p}$ are positions and velocities of the character, and $\phi \in [0,1]$ is a phase variable.
% Also, we add motion variables $c$, $l$, $v$ which are normalized crouch angle, stride length, and walking speed, respectively.
% Crouch angle is normalized using sine function, and stride length and walking speed are normalized to have zero mean and one standard deviation.
% Action is defined as target joint accelerations from PD control.
% We design the reward function $r$ as follows:
% \begin{equation}
%     r = ( {w}_{q}{r}_{q} + {w}_{v}{r}_{v} ){r}_{e} + {w}_{g}{r}_{g},    
% \end{equation}
  
% where ${r}_{q}$ is the reward term for tracking reference pose, ${r}_{v}$ is for tracking joint velocities of reference motion, ${r}_{e}$ is for imitation of end-effectors, and ${r}_{2}$ is for the goal encouraging to come back to the guide line after the push. We set the weight ${w}_{q} = 0.8$, ${w}_{v} = 0.1$, and ${w}_{g} = 0.1$. 


% \begin{equation}
%     r_q = exp(-\frac{\lVert q - q_{r} \rVert ^2}{\sigma_{q}} )
% \end{equation}


% \begin{equation}
%     r_v = exp(-\frac{\lVert \dot{q} - \dot{q}_{r} \rVert ^2}{\sigma_{v}} )
% \end{equation}

% \begin{equation}
%     r_g = exp(-\frac{\lVert  \rVert ^2}{\sigma_{g}} )
% \end{equation}





==> arXiv-Stability Analysis of Deep Control Policies for Biped Locomotion/chapters/push_recovery.tex <==

\section{Push-Recovery Experiments}

The primary goal of this research is to assess the robustness of deep policies in comparison with human subjects and pre-deep learning controllers. The study of Lee et al.~\shortcite{lee2015push} provides a reference for the comparison. We conduct push-recovery experiments with identical simulation setups to generate measurement data that can be directly compared to their results. 


\begin{figure} 
  \includegraphics[width=\linewidth]{figures/figure3.pdf}
  \caption{The setup for push-recovery experiments from top and lateral views. The blue line indicates the heading direction (Y axis).}
  \label{fig:push_recovery}
\end{figure}


The motion capture and measurement data from the previous study are available on their project webpage ~\cite{lee2015push}. The data set includes push-recovery experiments of 29 healthy adults (14 males and 15 females). The participants walked along a straight line with the choice of two speeds (normal/slow), two stride lengths (normal/short), and four levels of crouching (normal/20$^\circ$/30$^\circ$/60$^\circ$). The experimenter pushed the participants sideways to measure the maximal detour distance (see Figure~\ref{fig:push_recovery}). They also recorded a great deal of data including the height, weight, leg length, BMI of the participants, magnitude/timing/direction/duration of pushes, number of steps to maximal detour, detour of the first step, and push force normalized by height/weight/leg length. We refer the readers to the work of Lee et al.~\shortcite{lee2015push} for the details of the data acquisition process and specification.

Lee et al.~\shortcite{lee2015push} also performed statistical analysis on their data using a LMM (Linear Mixed Model) method and identified four significant factors (the level of crouch, walking speed, push timing and magnitude) that are correlated with maximal detour distance. Based on the analysis, they also performed comparisons between human and simulation experiments to see if simulated controllers are as robust as human balance strategies. Specifically, they adopted a Data-Driven Controller (DDC) by Lee et al.~\shortcite{lee2010data} for their experiments, which was designed before the advent of deep learning. Their experiments showed that the response pattern of the controller is qualitatively similar to how humans respond to external pushes, though the controller is not as robust as human walking yet.

In this paper, we conduct two sets of experiments. The first type of experiments is to faithfully reproduce the experiments of Lee et al.~\shortcite{lee2015push} with a new state-of-the-art biped locomotion simulation. Through the experiment, we would like to understand how deep policies compare with human walking and pre-deep-learning simulators. To do so, we generated a family of kinematic walking motions with stride lengths, walking speeds, crouch angles, and the magnitude/timing of pushes that match the distribution of human data (see Figure~\ref{fig:param_all}). The crouch angle is discrete, while all the other parameters are continuous and sampled from normal distributions. The push force in the simulation environment is applied to the shoulder and its magnitude is also sampled from the normal distribution of the human experiment data. The push timing is sampled between the left heel strike ($0\%$) and the subsequent right heel strike ($100\%$). Ten thousand push experiments were performed for each of four crouch levels. 

The second type of experiments is for assessing the implementation choices in DRL algorithms, such as random perturbation in learning, gait-specific versus gait-conditioned policies, and adaptive sampling. Since only DRL algorithms are compared with each other, we measure the success rate for evaluating the stability of control policies. An episode of simulation is considered successful if the biped withstands a push and keeps walking for 10 seconds afterwards while maintaining its balance. 

\begin{figure}
    \centering
    \includegraphics[width=.8\columnwidth]{figures/param_all}
    \caption{A family of walking motions with various walking speeds, stride lengths, and crouch angles.}
    \label{fig:param_all}
\end{figure}

There are several popular methods, such as maximum Lyapunov exponents and maximum Floquet multipliers~\cite{dingwell2000local}, for estimating the stability of dynamical systems. These methods quantify how the dynamical systems respond to small perturbations assuming strict periodicity. Small exponents or multipliers indicate that the system would return to a limit cycle. Human locomotion under disturbances is not a simple dynamical system since the control system is continuously modulated to maintain its balance. Its analysis often requires radical approximation of the dynamical system. In computer graphics, push-recovery stability is more popular since resilience against unexpected disturbances is closer to real-life notions of stability. Push-recovery stability quantifies how humans respond to impulsive perturbations. More specifically, maximum detour distances are useful if the experiment involves human participants who can cope with only moderate disturbances. The rate of success would be a better criterion under larger disturbances. There is no ultimate measure of dynamic stability. Assorted measures illuminate different aspects of gait stability. It is possible that a particular gait is very stable in one criterion but not in another.


 %We used institutional review board (IRB)-certified human data provided from the previous research \cite{lee2015push}. Quantified information extracted from push-recovery experiments for 29 healthy adult participants (14 males and 15 females) are contained in the data, which include body conditions and varieties of measured value of walking with a push.

%First, in order to compare the stability between the human and the DRL controller, the configuration for simulation experiments should be set to be the same as for human experiments. However, in human experiments, parameters such as stride length, walking speed, and magnitude/timing of push cannot be controlled as completely as in simulation. Therefore, we sampled the normal distribution of motion parameters of human data and let the controller mimic the modified motion with them.
% 먼저사람과 drl controller 간의 안정성을 비교하기 위해서는 사람 대상으로 실험했을 때와 최대한 동일하게 시뮬레이션 실험을 세팅하였다. 
% 사람의 걸음걸이에서 보속이나 보폭 등을 시뮬레이션처럼 일정하게 조절할 수 없다. 따라서 우리는 각 모션 파라미터 of 사람 데이터가 이루는 normal distribution 에서 sampling하여 이를 가지고 수정한 모션을 mimic하여 걷도록 하였다.  
% We sample motion parameter values using the normal distribution as the human data have the normal distribution.
%Push force is applied to the shoulder from the left and the push magnitude and timing are sampled according to the normal distribution of the human data. Timing of push is sampled between the left heel strike (0\%) and right heel strike (100\%) for 8-th step.
% human push 실험에서 했듯이 시뮬레이션에서도 push 실험을 했다. 왼쪽에서 캐릭터의 어깨 조인트를 밀고, 사람 데이터의 push timing과 magnitude data의 normal distribution 에서 값을 뽑아서 적용해서 밀었다.
% 이에 따라 수정한 모션을 레퍼런스 모션으로 준다. 그러면 이를 따라가는 시뮬레이션이 진행되는데, 이 때 사람 피실험자에게 해줬던 것처럼 미는 실험을 진행한다.
% 우리는 DRL을 사용하여 level of crouch (0, 20, 30, 60)에 따라서 각각 컨트롤러를 학습시켰으므로 우리는 네 개의 컨트롤러가 있다.
% level of crouch (0, 20, 30, 60) 마다 만 번의 push recovery test를 진행하여 성공한 tuple을 모은다.
% human 대상 실험에서는 shoulder를 밀었다. push는 보통 왼쪽 발만을 땅에 디디고 있을 때 왼쪽에서부터 가해지도록 했다.  
% push timing (single stance, double stance, \% of gait cycle)도 바꿔가며 실험했다.  
% human push 실험에서 했듯이 시뮬레이션에서도 push 실험을 했다. 왼쪽에서 캐릭터의 어깨 조인트를 밀고, 사람 데이터의 push timing과 magnitude data의 normal distribution 에서 값을 뽑아서 적용해서 밀었다.
% For the statistical analysis, plenty of data are needed, so we did ten thousand experiments for each DRL controller.
% 통계 분석을 위하여 충분히 많은 데이터를 얻기 위해, 각 컨트롤러당 만 번씩 실험을 했다. 

% To collect the experimental data from the simulation for comparison with human data, we used controllers parameterized with step length and walking speed which are sampled using adaptive method, training with push for each level of crouch. Ten thousand push recovery experiments were performed for each level of crouch.

% In the experiment for comparison between DRL controllers, the motion parameters were sampled with uniform distribution. 
% Because it is valid comparison for the controllers trained with two sampling methods (uniform and adaptive). 
% We use constant push force (100N). The experiment was run one thousand times for each controller.
% drl controller간의 비교를 위한 실험에서는 uniform distribution으로 motion parameter를 뽑아서 실험하였다. 
% training 시에 두 가지 Sampling 방법을 사용하는데, 실험 결과의 동등한 비교를 위해서 motion parameter를 uniform sampling을 하였다. 
% 각 컨트롤러 당 천 번씩 실험을 돌렸다.

%\subsection{Quantitative Measures for Stability}

%In many researches about biped control in graphics, methods applying push force or throwing balls or boxes to the character in simulation have used for proving the robustness. 
%However, when performing push recovery experiments on human subjects, it is dangerous to push humans with force large enough to fall down.
% When doing the push recovery experiment to the human subject, it is risky to push human with large force while there's no porblem in the simulation. 
%Therefore, in the previous study \cite{lee2015push}, they measure maximum detour distance after push, and use it as stability criterion. 
% 기존 연구 \cite{lee2015push}에서는 maximum detour distance를 측정하여 이를 안정성을 기준으로 삼았다.
% 시뮬레이션에서는 넘어질 때까지 밀 수 있지만, 사람 대상 실험에서는 위험하기 때문에 그럴 수 없다. 따라서 적당히 밀고, 얼마만큼 밀린 후 커버하는 데 얼마나 걸리는지를 MEASURE하는 것이 타당하다고 본 것. 
%We use detour distance measure to compare the human data with the experimental data from the DRL controller.
% 사람 데이터와 DRL controller의 실험데이터를 비교하기 위해 detour distance measure를 사용하기 했다.


%Next, we present a success rate as a quantitative measure to compare the stability between the controllers learned.
%In the previous study, because human experimental data has no failure case, they only used the successful simulation data, and failure cases were ruled out.
%However, when collecting simulation data, failure cases occur when the character falls down losing balance during the push-recovery experiment.
%We define success rate of push recovery experiment as a percentage of case where the simulated character walks straight along the guide line for 10 seconds after push force is applied.

% 다음으로, 우리는 학습한 총 8가지의 controllers 간의 안정성을 비교하기 위한 quantitative measure로 success rate를 제시하려고 한다. 기존 연구에서는 사람에 대해 push recovery experiment를 할 때 피험자가 넘어지지 않을 정도의 힘으로 밀었기 때문에, 실패한 경우는 배제되어 있다. 그러나 시뮬레이션 데이터를 모을 때는 실험 시에 캐릭터가 중심을 잡지 못하고 넘어진 failure case가 발생한다. Success rates는 총 실험한 횟수 중에 guide line 일직선으로 똑바로 걸어가는 캐릭터가 중간에 밀린 후, 다시 그 라인으로 돌아와서 10초간 넘어지지 않고 걸어가는 케이스들의 수를 백분율로 정의한다.


% \color{red}
% 이걸 언급하는 것이 이득일지, 실일지 모르겠고, discussion에 서술하는 것이 맞나 싶지만 ..
% 어쨌든 simulation results들을 detour distance로 안정성 비교하는 것이 fair하지 않다.
% data-driven method이기 때문에, 결국에는 기존 모션을 잘 따라가면 reward를 많이 받는데, push, no push training 결과만 비교해보면 no push distance가 훨씬 작다. 왜냐면 얘는 밀리는 것을 학습한 적이 없는 controller이기 때문에, 기존 모션을 많이 벗어나지 않도록 학습된 아이다. 그래서 실험에서 큰 힘으로 밀려서 많이 벗어나면 그냥 실패해버리고, 작은 힘으로 밀리면 기존 모션에서 많이 벗어나지 않은 채로 성공적으로 걷기 때문에, 성공률은 no push가 훨씬 적은데, 성공한 경우의  distance는 엄청 작게 나오는 것이다. 성공률만 보면 PUSH가 안정적인 거고, distance만 보면 no push가 안정적인 거다. 그래서 사실 distance만 살펴보는 것이 안정성을 평가하기에 좋은 measure인가 의문이 든다.  

% \color{black}

% The data used at the experiments are available at \url{http://mrl.snu.ac.kr/research/ProjectPushRecovery/}. 



% \subsection{Dataset for Camparison}
% % \subsection{Human Experiments and Previous Feedback controller}
% % 어떤 데이터인지 부가적인 설명 한줄 더?
% We used institutional review board (IRB)-certified human data provided from the previous research \cite{lee2015push}.
% Quantified information extracted from push-recovery experiments for 29 healthy adult participants (14 males and 15 females) are contained in the data, which include body conditions and varieties of measured value of walking with a push.
% % 기존의 피드백 컨트롤러로 생성된 데이터는 기존 연구에서 받아왔다. 
% % \color{red}
% % In the previous study, there was unnatural gait data collected in a way that subjects were asked to walk slowly or to walk in shorter steps deliberately. We excluded these data which disrupt expressing the natural distribution of human movement.
% % % 이전 연구에서 사람 데이터를 얻는 과정 중에 normal gait를 하는 subject에게 일부러 느리게 걷도록 하거나, 일부러 보폭을 줄여서 걷도록 주문한 unnatural 걸음 데이터가 있는데, 이를 제외한 데이터를 취급하기로 하였다. 사람의 자연스러운 움직임의 distribution을 표현하는데 저해되므로.
% % \color{black}
% For the data of the feedback controller, we also used data from the previous research \cite{lee2015push}.
% The data is generated by the controller proposed by Lee et al. ~\shortcite{lee2010data} with feedback parameters obtained by optimization.
% % cma로 노말 워킹에서 crouch 0도, 60도 모션을 가지고 먼저 feedback parameter를 구했다.
% % 이 때 push를 적용했다.
% % 그 결과 얻어진 컨트롤러로 push recovery experiment를 진행하여 시뮬레이션 데이터를 얻어냈다.
% % 이 때 walking parameters (crouch angle, step length, walking speed, push force, push timing)들을 normal distribution에서 random으로 뽑아내어 나온 모션을 트래킹하도록 하였다.
% The detailed information about the data acquisition process and specification are described in the paper \cite{lee2015push}.


==> arXiv-Stability Analysis of Deep Control Policies for Biped Locomotion/chapters/relatedwork.tex <==

\section{Related work}

\subsection{Physics-based Simulation and Control}

The design of biped controllers that produce realistic human walking has been a challenging subject in computer graphics.
The key challenge is designing a balancing mechanism, which is usually implemented as a feedback loop that adjusts the controller output (joint torques or PD target poses) based on its input (body state and environment information). A variety of control approaches has been explored to generate responsive and realistic human locomotion with diverse feedback mechanisms. Finite state machines equipped with manually-designed, intuitive feedback rules have been an effective approach in the early biped controller design~\cite{conf/siggraph/HodginsWBO95,yin2007simbicon}. 
%These approaches have demonstrated that manually-designed feedback rules followed by tuning a few coefficients could be an effective way of implementing a balancing mechanism. 
To mitigate the complexity of full-body dynamics, simplified dynamics models such as inverted pendulums have been used in controller design~\cite{kwon2010control, Coros:2010:GBW:1778765.1781156,tsai2009real,Mordatch:2010:SIGGRAPH,kwon_momentum-mapped_2017}.
% Feedback rules can be derived automatically from simplified dynamics models.

Data-driven (a.k.a. example-guided) approaches have been frequently used to improve the naturalness of simulated animations by adopting motion capture data as a reference to track~\cite{sok2007simulating,lee2010data,liu2012terrain,2016-TOG-controlGraphs}.
%, which is an effective approach to address unnatural stomping gaits often observed from the controllers based on finite state machines.
The balance mechanisms for data-driven controllers can be manually-crafted~\cite{lee2010data}, learned from a collection of example motions using a regression method~\cite{sok2007simulating}, or derived from a linear feedback policy using stochastic optimization and/or linear regression~\cite{liu2012terrain,2016-TOG-controlGraphs}.
%In this approach, balancing mechanisms are implemented by modulating reference motion data using SIMBICON-style feedback rules along with synchronizing contact timings~\cite{lee2010data}, choosing the best target pose among a number of optimized poses by a simple regression method~\cite{sok2007simulating}, or finding a linear feedback policy around motion clips using stochastic optimization or linear regression~\cite{liu2012terrain,2016-TOG-controlGraphs}.
Model predictive control (MPC) is used for synthesizing the full-body character animations in a physically plausible manner using reference motion data \cite{da2008simulation, hong2019physics}. Trajectory optimization is also employed to fulfill given tasks \cite{al2012trajectory, pan2018active, liu2018learning}. Many studies have utilized nonlinear optimization methods to  improve the robustness of controllers, or to explore control schemes for given tasks ~\cite{ye2010optimal, sok2007simulating,liu2012terrain,Lasa:2010:SIGGRAPH, Wang:2010:SIGGRAPH, wang2012optimizing}.

\subsection{DRL for Locomotion Control}

Recently, deep reinforcement learning has received significant attention and shown impressive improvements in the biped control problem. 
The control policy represented by a deep neural network can effectively achieve a feedback balancing mechanism in learning-based control.
% The feedback balancing mechanism is  called {\em control policy} in learning-based control and represented as a deep neural network. 
A variety of DRL algorithms has been proposed to learn control policies for biped locomotion~\cite{heess_emergence_2017, schulman2015high, yu2018learning}. Yu et al.~\shortcite{yu2018learning} proposed a mirror symmetry loss with curriculum learning to learn a locomotion policy without any reference data.

DRL algorithms can also take advantage of using motion capture data. Liu et al.~\shortcite{liu_learning_2017} used deep Q-learning to learn a scheduler that reorders short control fragments which are in charge of reproducing short motion segments. Peng et al.~\shortcite{peng_deeploco:_2017} presented a two-level hierarchical DRL-based control framework learned from short reference motion clips. They also presented a DRL method in their follow-up study to learn a control policy that imitates a given reference motion clip~\cite{2018-TOG-deepMimic}.
%One of the key ideas is to randomly select the initial state in the reference motion at the beginning of each episode, which allows the feedback mechanism to be trained efficiently for the character state around the reference motion.
Lee et al.~\shortcite{lee2019scalable} proposed a DRL-based controller for a muscle-actuated anatomical model.
Learning a control policy that exploits a set of reference motion data can be facilitated by recurrent neural networks~\cite{Park:2019} and a motion matching technique~\cite{bergamin2019drecon}.
Although the adoption of DRL in biped control has been very successful, few in-depth analysis of the characteristics of DRL-based controllers has been presented.
%We investigate the characteristics of a DRL-based controller and its variants in terms of push-recovery capability with different sets of gait parameters such as walking speed and stride length.

\subsection{Stability Analysis}

Gait and postural stability has been measured quantitatively using a waist-pull system~\cite{rogers2001lateral} and a movable platform~\cite{brauer2001interacting}, which can apply quantified perturbations to human subjects. In biomechanics, gait stability has been estimated using measures derived from nonlinear time-series analysis, such as Lyapunov exponents and Floquet multipliers~\cite{dingwell2000local}. The correlation of foot placement with balancing capability has been investigated in biomechanics and robotics~\cite{10.1115/1.4005462}. Wight et al.~\shortcite{10.1115/1.2815334} advocated Foot Placement Estimator (FPE) as a measure of balance for bipedal robots. %Lee et al.~\shortcite{lee2015push} postulated that foot placement plays a dominant role in gait stability.
In computer graphics, measuring the response to unexpected external pushes is a common criterion for estimating the resilience and robustness of controllers~\cite{yin2007simbicon,Mordatch:2010:SIGGRAPH,kwon_momentum-mapped_2017,lee2010data,2016-TOG-controlGraphs}.

% Tell a bit more about what Lee 2015 did, and in particular, what new this paper contributes 

% 특히, Lee et al.은 사람과 feedback 기반 제어 방식으로 시뮬레이션되는 캐릭터에 대한 밀림-회복 안정성을 통계적으로 분석하였다.
% 이 연구에서는, 사람이 보행 도중에 밀렸을 때 밀린 최대 거리를 안정성의 척도로 정하고, 사람을 직접 미는 실험과 이에 대한 통계적인 분석을 통해 밀린 거리에 영향을 미치는 보행 factor들을 찾아냈다.
% 그리고 이 보행 factor들이 simulated biped에도 영향을 미친다는 것을 보였다.
% 우리는 DeepRL 제어 방식으로 시뮬레이션 되는 캐릭터에 대한 밀림-회복 안정성을 사람 및 이전 feedback 기반 제어 방식으로 시뮬레이션 되는 캐릭터와 비교하였다.
% 거기에 더하여, 밀림-회복에 대한 success rate를 안정성의 척도로 사용하여 implementation choices in DRL algorithm 에 따른 안정성을 비교하였다.

Lee et al.~\shortcite{lee2015push} statistically analyzed the push-recovery stability of humans and that of simulated bipeds controlled by a hand-crafted feedback controller~\shortcite{lee2010data}.
Using maximum detour distance as a stability measure, they identified key gait factors (walking speed, level of crouching, push magnitude and timing) that affected the stability of human walking through statistical analysis. Their experimental setups are adopted in our simulation experiments and their human experiments serve as a reference of human vs simulation comparisons in our study.

%Based on their study, we compared the push-recovery stability of simulated biped using DRL control to humans and simulated bipeds using feedback control.
%Also, we assessed the gait stability according to the implementation choices in DRL algorithms by using push-recovery success rate as another stability measure.

% Lee et al.~\shortcite{lee2015push} statistically analyzed the push-recovery stability of humans and simulated bipeds and showed that the key gait factors that affect the stability of human walking also affect the stability of simulated walking.

This study begins with a question about how the characteristics of DRL-based controllers are similar or different compared to human walking and previous biped controllers. We aim to gain a deeper understanding and insight into how DRL achieves better stability in notoriously-challenging control problems.

%Lee et al. statistically analyzed the push experiments for human participants and a simulated character~\cite{lee2015push}.
%They found that the simulated character using a manually-designed linear feedback rules~\cite{lee2010data}, which is even applied only to the key joints such as hips, has the same gait factors as the human participants that affect their push-recovery capability.
% We began this study with the question of how similar or different characteristics of DRL-based controllers, which are considered to be more optimal feedback policies, are to traditional controllers.
% We aim to gain a  deeper understanding and insight into human locomotion and its push-recovery stability by comparing the stability of a deep policy network trained by a DRL algorithm with that of human participants and the previous controller using the manually-designed feedback rules. % using the same push-recovery stability measure.
% To understand the deep control policy in depth, we conduct more experiments and analyses on the variants of DRL-based control policies as well as their foot placement analysis.
% We try to find answers to the questions raised in Introduction from these comparisons and analyses.


% Researchers from various fields have analyzed gait and postural stability quantitatively from measured human movement.
% A waist-pull system \cite{rogers2001lateral} or movable platform \cite{brauer2001interacting} were proposed to apply quantified perturbation to human subject in standing pose to study postural stability. In biomechanics, gait stability is usually measured by kinematic variability such as Lyapunov exponents or Floquet multipliers~\cite{dingwell2000local}. Interestingly, the stability measured by these kinematic variability with changes in walking speed and stride length was reported as opposed to push-recovery stability~\cite{lee2015push}. The correlation of foot placement and balancing capability has been investigated in biomechanics and robotics~\cite{10.1115/1.2815334, 10.1115/1.4005462, 10.1115/1.4000193}.
% Wight et al. suggested Foot Placement Estimator (FPE) as a measure of balance for bipedal robots~\cite{10.1115/1.2815334}.
% Lee et al. described that when human walks, foot placement has a dominant role in balancing as well as in-place balancing~\cite{lee2015push}.


%런 애들은 어떤 거고 어떤 의미가 있는데, 주로 작은 섭동에 관련한 측정치들이었다.
% 트레드밀에서 당기는 실험이나 미는 실험들 한 것들 레퍼런스 달기.
%They used waist-pull system \cite{rogers2001lateral} or movable platform \cite{brauer2001interacting} to apply the perturbation to human subject, observe and analyze the reactions.

%Robotics researchers did push-recovery analysis for designing the exoskeleton \cite{kopitzsch2017optimization}.

%In animation field, there were relatively few endeavor to establish the standard to measure the stability of the controller quantitatively.
%There are diverse approaches for biped control as we described above. To evaluate the stability of the controller, researchers apply the external push to the character and see it can endure \cite{sok2007simulating, lee2010data, wang2012optimizing}. 
%They did change the environment \cite{lee2010data} or character's morphology.
%In researches using DRL controller, they also adopt the same way to prove the controller's robustness. They throw the boxes or ball to the character while walking \cite{2018-TOG-deepMimic, lee2019scalable}, change the environment (stairs, bumpy terrain) \cite{2018-TOG-deepMimic}, do retargeting \cite{yu2018learning}, or change the body segments (weakening muscle, using prosthetic leg) \cite{lee2019scalable}.
% 외부 섭동에 대해 robust하다는 것을 mild하게 보여주고 있다 공을 던진다던가, .
%These are methods to prove the stability qualitatively by showing the robust simulated results when something changes.   
% 무언가가 바뀌었을 때 이에 무너지지 않고 잘 걷는 것을 보여준다는 측면에서 qualitatively stable하다고도 말할 수 있으나, 부족한 감이 없지 않아 있다. 
% 여러가지 컨트롤 방법들이 연구되어 왔는데, 과연 이들을 분석할 기준, 방법들이 존재하는가에 대한 의문이 있다..
% However, there are lots of curiosity to be answered about the controller design.
% 안타깝게도 컨트롤러들의 성능에 대한 적절한 분석 기준이 없고, 이에 대한 연구들이 거의 없었다. 
%Lee et al made an effort for understanding the correlation between the human gait and the stability \cite{lee2015push}. They did push-recovery experiments using the feedback controller \cite{lee2010data} and analyzed the data compared the human's. They used detour distance as a stability measure under the external perturbation. At last, statistical analysis was possible by presenting quantitative criteria.

% 사람이 이족 보행 시에 foot placement가 밸런싱에 중요하다고 알려져 있다 \cite{10.1115/1.2815334, 10.1115/1.4005462, 10.1115/1.4000193}. 사람이 중심을 잡기 위해서 in-place balancing과 foot placement 이 두 가지 strategy를 혼용한다고 알려져 있다. 특히 이전 논문에서는 이족보행시에 foot placement가 dominant role을 한다고 서술하였다. 

% The push experiments, pushing a character by unexpected external pushes, are common method to demonstrate the resilience and robustness of  controllers~\cite{yin2007simbicon,Mordatch:2010:SIGGRAPH,kwon_momentum-mapped_2017,lee2010data,2016-TOG-controlGraphs}.
% Lee et al. statistically analyzed the push experiments for human participants and a simulated character~\cite{lee2015push}.
% They found that the simulated character using a manually-designed linear feedback rules~\cite{lee2010data}, which is even applied only to the key joints such as hips, has the same gait factors as the human participants that affect their push-recovery capability.
% We began this study with the question of how similar or different characteristics of DRL-based controllers, which are considered to be more optimal feedback policies, are to traditional controllers.
% We aim to gain a  deeper understanding and insight into human locomotion and its push-recovery stability by comparing the stability of a deep policy network trained by a DRL algorithm with that of human participants and the previous controller using the manually-designed feedback rules. % using the same push-recovery stability measure.
% To understand the deep control policy in depth, we conduct more experiments and analyses on the variants of DRL-based control policies as well as their foot placement analysis.
% We try to find answers to the questions raised in Introduction from these comparisons and analyses.

%This resembles the balancing process of real humans, which decide actions based on sensory inputs.

%\subsection{Previous Controllers}
% \color{red}
%%For decades, computer graphics researchers tried to build a biped controller which mimics the human walking as close as possible. 
%One approach is the feedback control. 
%Sok et al \cite{sok2007simulating} simulated biped walking with the regression and the controller can handle the external disturbance.
%% Gait simulation에서 중요한 factor가 두 가지가 있다고 했다. 자연스러운가, balancing 잘 하는가.
%넘어지지 않고 걷기 위해서는 balancing이 중요한데, 이를 위해서 phase별로 나눠서 feedback control하는 방법들을 사용하였다 \cite{yin2007simbicon}. 이 방법은 놀랍게 잘 되었지만, 아무래도 사람과 비슷한 느낌의 모션을 만들어내기는 힘들었다. 또한 다른 캐릭터나 다른 모션에 대해서 generalization이 힘들었다. 
%For achieving the naturalness of human movement, data-driven control is used \cite{lee2010data}.
%% 사람 움직임의 자연스러움을 얻기 위해서 data-driven simulation 방법들이 도입되었다 \cite{lee2010data}. 
%Feedback controllers with data-driven approach were done \cite{lee2010data, ye2010optimal, kwon2010control}.
%% 또는 최적화를 통하여 controller를 만드는 연구들도 있었다. 
%Another way to make a controller is optimization-based method \cite{ye2010optimal, wang2010optimizing, wang2012optimizing, al2012trajectory}. Many researchers believe that there are some principles when human moves. One of the popular claim is that human moves in energy efficient way. In optimization-based approach, they design the objective function using the prior knowledge or human insight, and optimized parameters. 그러나 이런 방법은 제한적이었고, 성능면에서 많이 나아지지도 않았다.
%trajectory optimization. 시간이 많이 걸리고. 
%환경이 달라지면 fragile 하였다. 


% \color{black}

%\subsection{Controllers using DRL}
%DRL learns from trial-and-error and its expressiveness is huge, so it has been used as a tool for designing the controller of a robot or a virtual character.

%In robotics society, passive walk robot is simulated \cite{mcgeer1990passive}. Mao et al \cite{mao2007reinforcement} used reinforcement learning to control the robot. Xie et al \cite{xie2018feedback} and Li et al \cite{li2019using} used DRL for controlling biped robot.

%In computer graphics area, DRL are widely used for producing the controller.
%DRL is used for synthesizing the motion from scratch in various study \cite{DBLP:journals/corr/DuanCHSA16, schulman2015high, yu2018learning}, but the results fall short of our expectation.
%Yu et al \cite{yu2018learning} used symmetry and low-energy as a reward function to train the network for walk without the reference motion. Although the resulting motion is stable and good compared with the previous results, but still far from the natural human walking. 
%How to design a reward function matters most in DRL framework, because the reward means to give the direction toward the goal. These approaches which use human insight or known principles for human movements can reach the limit blocked by various problems such as what to choose, and parameter tuning, etc. 
% rl에서는 reward function 디자인이 중요하다. 이것으로 어떤 골을 향해 가야하는지 컨트롤에 대한 방향을 제시하는 것이기 때문이다. 그러나 이 reward function design을 하려고 하면 human insight에 기댈 수 밖에 없고, 이것저것 갖다대다보면 지저분해지는데, 또 그렇다고 막 성능이 좋아지지도 않는 현상이 발생한다.
%To mitigate this problem, Peng et al \cite{2018-TOG-deepMimic} used data-driven approach with DRL to simulate human locomotion. The controller is trained to mimic the reference motion data and they demonstrate basic skills and dynamic skills like flips and spins. By applying the two critical techniques, one is to choose the initial state randomly and the other is early termination during training, they can accomplish making the robust controller using DRL. Lee et al \cite{lee2019scalable} used musculoskeletal model and simulated various human locomotion. They can also simulate the pathological gait by changing the muscle properties. Training a network that can control multiple reference data also be possible with the combination of DRL and motion graph (RNN) or motion matching \cite{Park:2019, bergamin2019drecon}.

% We used the simulation framework proposed by Lee et al \cite{lee2019scalable} to obtain the walking motion data from DRL controller. 

%\subsection{Stability Analysis Method}



% \subsection{Character Modeling}

% Humanoid character models used in biped simulations have evolved constantly. Early models are very simple, robot-like design with a few body parts articulated with motor-joints, such as lower-limb model in 2D \cite{sok2007simulating, yin2007simbicon}.  
% % biped simulation을 위하여 사용되어 온 character model은 계속 발전하여 왔다. 처음에는 전형적인 로봇 같이 조인트 토크로 actuate 되는 모델이 많았다. 하체만 있거나 2d에서 시뮬레이션하는 모델들. 또는 inverted pendulum과 같이 simplify된 모델들을 사용하였다. 간단해서 컨트롤이 쉬웠기 때문이다.
% The simpler the model, the easier it is to control.
% In succession, full body joint-torque models in 3D were introduced \cite{lee2010data, wang2010optimizing}.
% Inverted pendulum model is used for balancing by adjusting the center-of-mass \cite{tsai2009real, kwon2010control, Coros:2010:GBW:1778765.1781156}.

% However, these kinds of model can yield somewhat rustic motions because it has structural limitations to reproducing realistic movements such as humans. Necessity of more exquisite human body modeling for the simulation of the human locomotion has been raised. As a result, the musculoskeletal human body models were used.  
% % 그러나 이런 모델들로 나온 모션들은 실제 환경에서의 사람의 움직임과는 동떨어져 보였고, 사람의 움직임을 사실적으로 재현하기 위해 더 복잡한 사람과 닮은 캐릭터들을 만들어내는 모델링 연구들이 진행되었다. 
% These models are actuated with the joint torques which are the net force generated by adjacent musculotendon units.  
% Wang et al \cite{wang2012optimizing} used eight major muscles in the lower-body to simulate human walking. Lee et al \cite{lee2014locomotion} and Lee et al \cite{lee2019scalable} used full-body humanoid characters having 120 and 284 line muscles for simulating various human movement. By using the model with the bone attached muscles, pathological gaits caused by muscle deficiency can be generated.
% % 기존의 조인트 토크로 움직이던 관절들이 사람이 실제 관절을 움질일 때처럼 근육에서 발생된 힘들을 합으로 조인트들을 움직이는 식의 musculoskeletal model \cite{wang2012optimizing, lee2014locomotion, lee2019scalable}들이 만들어졌다. 
% % 이 연구들로 인해서 어떠어떠한 것이 가능해졌다.

% % Modeling studies on specific body parts have also been conducted. In terms of a human foot, one important body part in gait, most previous studies assumed the foot as one or two segment \cite{lee2010data, wang2010optimizing}. To replace the simple foot model, soft foot model \cite{Jain:2011:CPC:2070781.2024197} or multi-segment foot model \cite{park2018multi, lee2019scalable} were proposed.
% % 풀바디 디자인의발전 말고도 사람의 걸음걸이에 중요한 신체 부분이 바로 발인데, 기존 대부분의 연구들에서는 발을 하나나 두 개의 덩어리로 놓고 연구해왔다. simple foot model \cite{lee2010data, wang2010optimizing}. 이를 대체하기 위해 soft foot model \cite{Jain:2011:CPC:2070781.2024197} and multi segment foot model \cite{park2018multi} 과 같은 모델들 연구도 나왔다.

==> arXiv-Stability Analysis of Deep Control Policies for Biped Locomotion/chapters/results.tex <==

\section{Analysis and Results}

We used Intel® Core™ i9-9900K CPU @ 3.60GHz (8 cores) for training. Training takes about 24 hours for gait-specific policies, and 40 to 50 hours for gait-conditioned policies. The neural network for all DRL controllers consists of three fully connected layers with 256 nodes. The network is updated whenever 8192 experience tuples are collected with 256 batch size. We used R (version 3.6.1) for the statistical analysis. 

In our experiments, we compared the push-recovery capabilities of human participants (Human), a data-driven controller (DDC) with hand-crafted feedback laws~\cite{lee2010data}, DRL gait-specific policies (DRL-specific), and DRL gait-conditioned policies with two continuous parameters (walking speed and stride length) and one discrete parameter (crouch angle). We denote gait-conditioned policies (see Table~\ref{tab:types_of_policies}) learned with and without adaptive sampling by DRL-A and DRL-B, respectively. DRL-specific*, DRL-A*, and DRL-B* are policies learned with unexpected disturbances in the learning phase.

\begin{table}
\caption{The name of each control policy. An asterisk means that the policy is trained with push, and -A means that adaptive sampling method is applied in the training.}
\centering
\begin{tabular}{ccc}
\toprule
                  & With push        & Without push \\
\midrule
Adaptive sampling &   DRL-A*         &   DRL-A      \\
\midrule
Uniform sampling  &   DRL-B*         &   DRL-B      \\
\bottomrule
\end{tabular}

\label{tab:types_of_policies}
\end{table}


\begin{table}
\caption{The means and standard deviations of factors in human experiments. The push magnitude is normalized by weight.}
\begin{tabular}{clcc}
\toprule
    \multicolumn{2}{l}{Experimental factor}       & Mean      & Std   \\ \midrule
Walking   &  Normal                               & 0.994     & 0.263 \\
speed     &  Crouch $20\,^{\circ}$                & 0.808     & 0.210 \\
(m/s)     &  Crouch $30\,^{\circ}$                & 0.788     & 0.221 \\
          &  Crouch $60\,^{\circ}$                & 0.744     & 0.228 \\ \midrule
Stride    &  Normal                               & 1.126     & 0.180 \\
length    &  Crouch $20\,^{\circ}$                & 0.953     & 0.158 \\
(m/s)     &  Crouch $30\,^{\circ}$                & 0.916     & 0.167 \\ 
          &  Crouch $60\,^{\circ}$                & 0.876     & 0.168 \\ \midrule
\multicolumn{2}{l}{Push magnitude (N$\cdot$s/kg)} & 0.535     & 0.096 \\ \midrule
\multicolumn{2}{l}{Push timing (\%)}              & 34.0      & 21.0  \\ 
\bottomrule
\end{tabular}
\bigskip\centering
\label{tab:human_data_mean}
\end{table}

The gait parameter domains for learning gait-conditioned policies are decided from human data (see Table~\ref{tab:human_data_mean}). More precisely, at the beginning of every episode in the learning process, gait parameters are sampled uniformly (for DRL-B and DRL-B*) or adaptively (for DRL-A and DRL-A*) in the region within a certain Mahalanobis distance $t$. We chose the value of $t$ to make the sampling region be 95\% confidence region. Note that the walking speed and stride length are correlated, and the correlation coefficient for each crouch walking ranges from 0.67 to 0.83.
For the training of control policies (DRL-specific*, DRL-A*, and DRL-B*) under the circumstance where external pushes are exploited, the simulated character is pushed for 0.2 seconds from the left or the right randomly.
The push direction always matches the stance leg. So, the push from the left happens when the left leg is in stance and vice versa. The magnitude and timing of pushes are sampled to match the distributions in the human experiment data (Table~\ref{tab:human_data_mean}). The push magnitudes were mostly in the range of 100N to 300N.
% For training controllers with push such as DRL-base*, DRL-A*, and DRL-B*, we push the simulated character for 0.2 seconds from the left or the right randomly.
% the simulated character pushed for 0.2 seconds to push the biped sideways from left or right.
%Note that we matched the push direction with the leg that entered the stance phase.
% The sides of the stance foot and push are the same.
%For example, the biped is pushed from the left when the left leg is in the stance phase. The push magnitude and timing are determined by human data (Table~\ref{tab:human_data_mean}). The magnitude of the pushes was mostly in the range of 100N to 300N in our setting.

\subsection{Human vs Simulation}

\color{red} 
% 5장 subsection 모두 두괄식으로 설명할 것!
% The locomotion policies learned by DRL achieved a closer metric (maximum detour distance) to real human data, compared to other methods.

%To figure out the stability of the control policies using DRL, we compared push-recovery experiment results of human data, DDC, and DRL in respect of maxmium detour distance. As a result, our parametric policies can achieve comparable results to human data, and superior results to DDC (Figure~\ref{fig:distance_box_plot_each}). 

\color{black}

The statistics of gait factors in human experiments are shown in Table~\ref{tab:human_data_mean}. The trials in human data are classified into two groups: {\em Group 1} and {\em Group 2}. The participants in {\em Group 1} trials recovered their balance in a single step, and thus the detour distance peaked in the step. Most of the participants recovered their balance within three balance-correcting steps except for a few outliers. They took more than one step when they experienced mild difficulty. In the outliers, participants panicked by unexpected pushes and failed to return to the line. The {\em Group 2} includes all trials except for the outliers.


\begin{figure}
  \includegraphics[width=\columnwidth]{figures/graph_distance.pdf}
  \caption{Box plots of maximum detour distance in Group 1 (left) and Group 2 (right). The horizontal line in the middle of each boxplot means median, and colored area represents from 25\% to 75\% of the data.}
  \label{fig:distance_box_plot_each}
\end{figure}


In Figure~\ref{fig:distance_box_plot_each}, we compare the maximum detour distances of Human, DDC, DRL-B*, and DRL-A*. The results of Human and DDC experiments were taken from the work of Lee et al.~\shortcite{lee2015push}. The simulation experiments were designed to reproduce the human experiments with setups and data distributions carefully tuned to match the target experiments. The only difference is that we can collect far more trial data by simulation. 
The {\em Group 1} of Human, DDC, DRL-B*, and DRL-A* include 228, 3858, 4851, and 16036 trials, respectively, and the {\em Group 2} includes 450, 13707, 20534, and 27993 trials, respectively. The comparison graph shows that DRL-B* and DRL-A* are clearly superior to DDC and comparable to human participants. 


% \begin{table}
% \caption{The success rates (\%) of parametric policies. }
% \begin{tabular}{lccccc}
% \toprule
%                         &   DRL-B*  &  DRL-A*  & DRL-B   & DRL-A   \\ \midrule
% Normal                  &   43.3   &  64.0   &   4.2   &   3.0   \\ 
% Crouch $20\,^{\circ}$   &   63.4   &  72.4   &  10.9   &   3.1   \\ 
% Crouch $30\,^{\circ}$   &   66.3   &  78.6   &   8.7   &  10.1   \\ 
% Crouch $60\,^{\circ}$   &   32.3   &  64.9   &   3.8   &  14.4   \\ 
% \bottomrule
% \end{tabular}
% \bigskip\centering
% \label{tab:Sampling_success_rate}
% \end{table}

\begin{figure}
  \includegraphics[width=\columnwidth]{figures/table2_graph.pdf}
  \caption{The success rates (\%) of gait-conditioned policies. }
  \label{fig:Sampling_success_rate}
\end{figure}


It was empirically verified in the previous study that crouch walking is more stable than normal walking in Human and DDC experiments. In particular, $30^\circ$-crouch walking was the most stable. This postulation agrees with our intuition that lowering down the CoM improves the gait stability. Although the detour distance measurements of DRL-B* and DRL-A* do not follow this trend, the success rate experiments agree with the postulation. Graph~\ref{fig:Sampling_success_rate} shows that both DRL-B* and DRL-A* are more robust with 20$^\circ$/30$^\circ$-crouch walking than normal and 60$^\circ$-crouch walking. $30^\circ$-crouch walking was the most robust in terms of the success rate.

%Our DRL-B* experiment also shows a similar trend except that $60^\circ$-crouch walking is more stable than $30^\circ$-crouch walking. It is strenuous for human participants to walk in $60^\circ$ crouching. $60^\circ$-crouch walking is less stable probably due to fatigueness, which is not implemented in our DRL algorithms. The simulated bipeds never get tired and maintain it balance capabilities even in strenuous tasks and situations.


\begin{table}
\caption{Type 3 tests of the fixed effects (level of crouch, walking speed, magnitude/timing of push) on the detour distance. Significant values ($p < 0.05$) are shown in bold.}
\resizebox{\columnwidth}{!}
{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{}} & \multicolumn{8}{c|}{Type 3 Tests for fixed effects}                                                                                               \\ \cline{3-10} 
\multicolumn{2}{|c|}{}                  & \multicolumn{2}{c|}{Level of Crouch} & \multicolumn{2}{c|}{Push Magnitude} & \multicolumn{2}{c|}{Walking Speed} & \multicolumn{2}{c|}{Push Timing} \\ \cline{3-10}
\multicolumn{2}{|c|}{}   & $F_{c}$  & \multicolumn{1}{c|}{$p_{c}$}   & $F_{f}$  & \multicolumn{1}{c|}{$p_{f}$} & \multicolumn{1}{c|}{$F_{s}$} & \multicolumn{1}{c|}{$p_{s}$} & \multicolumn{1}{c|}{$F_{t}$} & \multicolumn{1}{c|}{$p_{t}$} \\ \hline\hline
% Group1
\multirow{4}{*}{Group 1}& Human & \textbf{17.49} & \textbf{<.0001} & \textbf{13.42} & \textbf{0.0003} & 2.68 & 0.1098 & \textbf{14.35} & \textbf{<.0001}   \\ \cline{2-10} 
                    & DDC   & \textbf{30.06} & \textbf{<.0001} & \textbf{17546}  & \textbf{<.0001 } & \textbf{106.6} & \textbf{<.0001} & \textbf{463.4} & \textbf{<.0001}  \\ \cline{2-10} 
                        & DRL-A* & \textbf{196.5} & \textbf{<.0001} & \textbf{11791} & \textbf{<.0001} & \textbf{4536} & \textbf{<.0001} & \textbf{363.5} & \textbf{<.0001}  \\ \cline{2-10} 
                        & DRL-B* & \textbf{768.7} & \textbf{<.0001} & \textbf{3022} & \textbf{<.0001} & \textbf{625.6} & \textbf{<.0001} & \textbf{130.0} & \textbf{<.0001}  \\ 
                        \hline\hline
% Group2                       
\multirow{4}{*}{Group 2}& Human & \textbf{8.35} & \textbf{<.0001} & 0.01 & 0.9297 & 0.03 & 0.8578 & \textbf{3.94} & \textbf{0.0479}  \\ \cline{2-10} 
                        & DDC   & \textbf{88.34} & \textbf{<.0001} & \textbf{19103} & \textbf{<.0001} & \textbf{371} & \textbf{<.0001} & \textbf{225.8} & \textbf{<.0001} \\ \cline{2-10}
                        & DRL-A*& \textbf{7.857} & \textbf{0.0051} & \textbf{12427} & \textbf{<.0001} & \textbf{251.8} & \textbf{<.0001} &\textbf{2329} & \textbf{<.0001} \\ \cline{2-10}
                        & DRL-B*& \textbf{575.6} & \textbf{<.0001} & \textbf{10937} & \textbf{<.0001} & \textbf{57.53} & \textbf{<.0001} &\textbf{331.6} & \textbf{<.0001}            \\ \hline
\end{tabular}
}
% \vspace*{5mm}
\label{table:lmm1}
\end{table}


Table ~\ref{table:lmm1} shows the results of Type 3 tests, which shows the fixed effects of level of crouch, walking speed, magnitude/timing of push on the detour distance. The tests confirm that all factors that were proven to be significant in the human experiments are also significant ($p<0.05$) in the DRL experiments.

% all factors except the timing of push are significant (p < 0.05) in DRL simulation results (Table ~\ref{table:lmm1}). 
% In the previous study, the less the detour distance, the later push timing in Group 1, so later push timing is more stable. While in our results, push timing has no significance with detour distance.


% \begin{table}
% \bigskip\centering
% \caption{The success rate (2 depth) of baseline and parametric policies of $30^\circ$-crouch walking. Mean parameter values are shown in gray.}
% %\resizebox{\columnwidth}{!}
% {
% \begin{tabular}{cccccccc}
% \toprule
%  Walking    &   Stride    &  DRL-base*  &   DRL-B*       &  DRL-A*      \\
% speed (m/s) &  length (m) &   (\%)      &   (\%)         &    (\%)      \\ \midrule
% %0.35        &	0.58       &   72.0      &                &              \\ 
% %0.46        &	0.67       &   90.9      &     fail       &    fail      \\ 
% 0.57        &	0.75      &   88.4      &      5.1       &    46.8     \\ 
% 0.68        &	0.83      &   88.2      &     85.9       &    55.6     \\ 
% \cellcolor[HTML]{D3D3D3}0.79&\cellcolor[HTML]{D3D3D3}0.92&   92.1      &     92.2       &    79.8     \\ 
% 0.90        &	1.00      &   87.6      &     86.5       &    97.5     \\ 
% 1.01        &	1.08      &   85.3      &     85.1       &    92.1     \\ 
% 1.12        &	1.17      &   97.3      &      0.0       &    71.9     \\ 
% 1.23        &	1.25      &   95.6      &      0.0       &    55.1     \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:policy_comparison_2depth}
% \end{table}

% \begin{table}
% \bigskip\centering
% \caption{\color{red} (NORMAL GAIT conducting experiment....) \color{black} The success rates of baseline and parametric policies of normal walking. Mean parameter values are shown in gray. {\em Fail} indicates that a control policy was unable to learn the walking motion that has the corresponding walking speed and stride length.}
% %\resizebox{\columnwidth}{!}
% {
% \begin{tabular}{cccccccc}
% \toprule
%  Walking                    &   Stride                   &  DRL-base*  &   DRL-B*       &  DRL-A*      \\
% speed (m/s)                 &  length (m)                &   (\%)      &   (\%)         &    (\%)      \\ \midrule
% 0.46                        &	0.77                     &             &    fail        &              \\ 
% 0.60                        &	0.86                     &             &    56.8        &               \\ 
% 0.73                        &	0.95                     &             &    73.3        &               \\ 
% 0.88                        &	1.04                     &             &    72.9        &               \\ 
% \cellcolor[HTML]{D3D3D3}0.99&\cellcolor[HTML]{D3D3D3}1.13&             &    87.5        &           \\ 
% 1.13                        &	1.22                     &    93.8     &    92.8        &               \\ 
% 1.25                        &	1.30                     &    88.5     &    91.1        &               \\ 
% 1.39                        &	1.40                     &    85.8     &    87.0        &               \\ 
% 1.52                        &	1.49                     &             &    76.7        &               \\
% %1.65                        &	1.58                     &             &    fail        &               \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:policy_comparison}
% \end{table}


% \begin{table}
% \bigskip\centering
% \caption{The success rates of baseline and parametric policies of $30^\circ$-crouch walking. Mean parameter values are shown in bold. {\em Fail} indicates that a control policy was unable to learn the walking motion that has the corresponding walking speed and stride length.}
% %\resizebox{\columnwidth}{!}
% {
% \begin{tabular}{cccccccc}
% \toprule
%  Walking    &   Stride    &  DRL-base*  &   DRL-B*       &  DRL-A*      \\
% speed (m/s) &  length (m) &   (\%)      &   (\%)         &    (\%)      \\ \midrule
% %0.35        &	0.58       &   72.0      &                &              \\ 
% 0.46        &	0.67       &   90.9      &     {\em fail}     &    49.9     \\ 
% 0.57        &	0.75      &   88.4      &     89.6        &   88.0     \\ 
% 0.68        &	0.83      &   88.2      &     83.1      &    89.8      \\ 
% \textbf{0.79}&\textbf{0.92}&   92.1      &     92.4       &    86.7     \\ 
% 0.90        &	1.00      &   87.6      &     96.3      &    93.7     \\ 
% 1.01        &	1.08      &   85.3      &     98.2      &    91.1     \\ 
% 1.12        &	1.17      &   97.3      &     90.7      &    91.7     \\ 
% 1.23        &	1.25      &   95.6      &     70.0      &    85.6     \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:policy_comparison}
% \end{table}

\begin{figure}
  \includegraphics[width=\columnwidth]{figures/table4_graph.pdf}
  \caption{The success rates of gait-specific and gait-conditioned policies of $30^\circ$-crouch walking. Mean parameter values are shown in bold. We did not plot a {\em fail} case where a control policy was unable to learn the walking motion with the corresponding walking speed and stride length.}
  \label{fig:policy_comparison}
\end{figure}

\subsection{Comparison of Control Policies}

% \color{red}
% We proposed gait-conditioned policies which can deal with a wide range of gait parameter domain. During training, push force is randomly applied to increase the robustness against the external force. Gait-conditioned policies can use adaptive sampling (DRL-A*) or not (DRL-B*). We compared the push-recovery experiment results of each control method (DRL-A* and DRL-B*) and gait-specific policies (DRL-base*) in terms of success rate (Figure~\ref{fig:policy_comparison}).
% When the gait parameters are sampled near the mean values, success rates of DRL-A*, DRL-B*, and DRL-base* are evenly high. However, DRL-A* outperforms DRL-B* when choosing the gait parameter away from the mean values (Figure ~\ref{fig:sampling_plot}).
% % 여러가지 컨트롤 팔러시를 조건을 바꿔가면서 트레이닝해놨는데, 이들 간의 stability 도 비교해 볼 수 있다. We trained several control policies, DRL-base*, DRL-A*, DRL-B*, DRL-A, and DRL-B. Adaptive sampling을 사용한 DRL-A*가 더넓은 파라미터 도메인을 커버할 수 있음을 확인하였다 (Figure ~\ref{fig:sampling_plot}).  

  
% \color{black}

Gait-specific policies DRL-specific* supposedly outperform gait-conditioned policies DRL-A* and DRL-B* since the scope of the gait-specific policy focuses on a single reference trajectory, while the gait-conditioned policies have to cope with a continuous spectrum of parametric domains. Specifically, the domain $[\mu_s-1.5\sigma_s,\mu_s+2\sigma_s]\times [\mu_l-1.5\sigma_l,\mu_l+2\sigma_l]$ is explored in our experiments, where $\mu_s$ and $\mu_l$ are the average walking speed and stride length, respectively, in the human experiments. $\sigma_s$ and $\sigma_l$ are their standard derivations. The use of an asymmetric domain is related to the perception plausibility of motion editing. Edited character animations that walk slower than a reference are more likely to look unnatural than animations that walk faster than the reference~\cite{vicovaro_2014}.

\begin{figure}
  \includegraphics[width=\columnwidth]{figures/sampling_comparison_plot.pdf}
  \caption{The parameter coverage of successful episodes. Each ellipse represents a 98\% confidence region.}
  \label{fig:sampling_plot}
\end{figure}

We conducted push-recovery experiments of 1000 trials for each of the three policies. Push forces are drawn from a normal distribution with a mean of 200N and a standard derivation of 35N (see Figure~\ref{fig:policy_comparison}). A family of motion clips were generated to learn DRL-specific* polices. The stability of each gait-specific policy learned for a particular walking speed and a stride length is comparable to the stability of DRL-B* near the mean values, but clearly outperforms when the samples are away from the means. It means that na{\"i}ve parametric learning can deal with only a narrow range of the parametric domain. Adaptive sampling of DRL-A* improves the stability at the corners of the domain and consequently learns a policy practically usable over the entire domain within a modest computational time. Figure~\ref{fig:sampling_plot} depicts the parametric coverage of successful episodes. The coverage of DRL-A* is wider than the coverage of DRL-B*. It means that DRL-A* can better deal with slow walking (narrow strides) and fast walking (wide strides), while DRL-B* is effective only at mid ranges. 

Deciding the number of hidden layers of the policy network depends on the dimension and size of the action, state, and parameter spaces. In practice, the number of layers and the number of nodes in each layer are important hyper-parameters to tune empirically. In our experiments, we tested with two, three, and four hidden layers and found that learning was the most successful with three layers.
% (see Table~\ref{tab:network_layer_success_rate}). 


% \begin{table}
% \caption{The success rates (\%) of DRL-A* with the number of hidden layers in the policy networks.}
% \begin{tabular}{lccccc}
% \toprule
%                         &   2 layers    &   3 layers   &   4 layers    \\ \midrule
% Normal                  &    32.8       &    64.0     &     40.2      \\ 
% Crouch $20\,^{\circ}$   &    64.5       &    72.4     &     64.0      \\ 
% Crouch $30\,^{\circ}$   &    69.2       &    78.6     &     72.6      \\ 
% Crouch $60\,^{\circ}$   &    49.3       &    64.9     &     30.0      \\ 
% \bottomrule
% \end{tabular}
% \bigskip\centering
% \label{tab:network_layer_success_rate}
% \end{table}


\subsection{Foot Placement Analysis}

\begin{figure*}
    \begin{subfigure}{.325\textwidth}
      \centering
      % include second image
      \includegraphics[width=\linewidth]{figures/human_foot_placement_2d_fixed_length_speed_zerofoot_origin_3depth_normal.pdf}  
      \caption{Human data (Normal)}
      \label{fig:foot_placement_human}
    \end{subfigure}
    % \vskip\baselineskip
    \begin{subfigure}{.325\textwidth}
      \centering
      % include third image
    %   \includegraphics[width=\linewidth]{figures/foot_placement_depth3_adaptive_normal.pdf}  
    %   \includegraphics[width=\linewidth]{figures/foot_placement_2d_fixed_length_speed_zerofoot_origin_depth3_adative_normal_push_4sca_legend.pdf}  
    \includegraphics[width=\linewidth]{figures/sca_b.png}
      \caption{DRL-A* (Normal)}
      \label{fig:foot_placement_push}
    \end{subfigure}
    \begin{subfigure}{.325\textwidth}
      \centering
      % include fourth image
    %   \includegraphics[width=\linewidth]{figures/foot_placement_depth3_adaptive_normal_nopush.pdf}  
      \includegraphics[width=\linewidth]{figures/sca_c.png}
      \caption{DRL-A (Normal)}
      \label{fig:foot_placement_nopush}
      
    \end{subfigure}
    \vskip\baselineskip
        \begin{subfigure}{.325\textwidth}
      \centering
      % include second image
      \includegraphics[width=\linewidth]{figures/human_foot_placement_2d_fixed_length_speed_zerofoot_origin.pdf}  
      \caption{Human data ($30^{\circ}$-crouch)}
      \label{fig:foot_placement_human_30deg}
    \end{subfigure}
    % \vskip\baselineskip
    \begin{subfigure}{.325\textwidth}
      \centering
      % include third image
      \includegraphics[width=\linewidth]{figures/foot_placement_depth3_adaptive_crouch30.pdf}  
      \caption{DRL-A* ($30^{\circ}$-crouch)}
      \label{fig:foot_placement_push_30deg}
    \end{subfigure}
    \begin{subfigure}{.325\textwidth}
      \centering
      % include fourth image
      \includegraphics[width=\linewidth]{figures/foot_placement_depth3_adaptive_crouch30_nopush.pdf}
      \caption{DRL-A ($30^{\circ}$-crouch)}
      \label{fig:foot_placement_nopush_30deg}
    \end{subfigure}
    
    \caption{Foot placement plots. All foot placements are overlaid in the coordinate system. Green diamonds are the footprints to step on in the absence of external disturbances. Pre-push stance footprints are indicated by magenta dots or magenta diamonds. The blue and green dots represent the first post-push footprints of {\em Group 1} and {\em Group 2} - {\em Group 1} in successful episodes, respectively.
    The red dots are those of unsuccessful balance recovery episodes.
 The x-axis and y-axis are lateral and moving directions. The footprints are classified into intervals $(0\%, 20\%, 40\%, 60\%, 80\%, 100\%)$ of push timing indicated by black dotted curves.
 Note that each origin of the coordinates of human data is the mean of stance foot positions.}
    \label{fig:foot_placement_fixed_speed_step_length}
\end{figure*}

It has been previously postulated that balancing strategies based on foot placements play a dominant role in dynamic walking. We hypothesized that deep policies learn to smartly choose post-push footholds to recover balance within a few steps. 
% \color{red}
% We plotted the footsteps after pushing the character. After analyzing the footstep patterns, we found that control policy DRL-A *, training under the random external push forces, can learn to balance by stepping back more than when not pushed, which is similar patterns of human (See Figure~\ref{fig:foot_placement_human} and ~\ref{fig:foot_placement_push}). 
% % Also, the earlier the push timing is, the higher chance to balance.   
% \color{black}
We conducted push-recovery experiments with four deep policies DRL-A, DRL-B, DRL-A*, and DRL-B*. In each trial, the simulated biped was pushed from the left during its left foot in stance and took the next step on the right to recover its balance. Figure~\ref{fig:foot_placement_fixed_speed_step_length} shows that the stability of control policies are characterized by the pattern of post-push foot placements, which are plotted with respect to the reference footprint to step on if there are no disturbances. The push magnitude and timing are randomly sampled, while the walking speed, stride length, and crouch angle are fixed. Push magnitudes are sampled from a normal distribution with a mean of $200N$ and a standard derivation of $35N$. Push timings are sampled from another normal distribution of a mean of $34\%$ and a standard deviation of $21\%$.

We used 158 normal gait data, and 22 30$^\circ$-crouch gait data . 
% The human data include 158 normal gaits and 22 crouch gaits (30$^\circ$). 
Note that the human data were collected from many participants under varied conditions and thus necessarily noisy, while the simulation data were collected in a controlled simulation setup. Therefore, the side-by-side direct comparison is meaningless, but the data should be interpreted qualitatively. In the human data (Figure~\ref{fig:foot_placement_human}, \ref{fig:foot_placement_human_30deg}), the disturbed swing foot tends to land behind (in the y-axis) the undisturbed step position. It means that human participants tend to slow down temporarily to cope with lateral disturbances. The success rate of DRL-A is very low ($3.0\%$ for normal walking and $10.1\%$ for 30$^\circ$-crouch walking), and the post-push footholds of successful trials are all at nearly the same y-coordinate as the undisturbed reference step position since DRL-A did not learn how to cope with disturbances. Unlike DRL-A, DRL-A* exploited uncertainty in the learning phase and learned to adjust its step length (shorter in the y-axis) similarly to human balance strategies. 

The foot placement graphs in Figure~\ref{fig:foot_placement_fixed_speed_step_length} also show that post-push step positions are closely correlated with push timing. The push may occur in either a double-stance phase $[0\%,20\%]$ or a swing phase $[20\%,100\%]$. The push at the early swing phase allows the walker to have a sufficient time to move its leg to an appropriate position for balance recovery, while the push at the late swing phase forces the walker to put the swing foot down rapidly with little time for control. Therefore, control policies are more resilient to early-swing pushes than late-swing pushes. Note that maximum detour distances are shorter (can be interpreted as more resilient) with later-swing pushes, which seems contradictory to the proposition based on the success rate. As we discussed before, there is no ultimate criterion for resilience and gait stability. The notion of stability can be characterized richly by a mixture of measures.
For example, Figure~\ref{fig:foot_placement_fixed_speed_step_length} shows that the post-push step positions tend to be farther from the undisturbed reference step position as the timing of the push is earlier (the 20\% curve is farther than the 60\% curve from the reference position), but the success rate for early pushes are higher than late pushes (the ratio of blue and green dots in the <20\% push timing region is higher than that of the 40\%--60\% region).

As shown in Figure~\ref{fig:foot_placement_fixed_speed_step_length}, the successful post-push steps of normal gaits are mostly placed less in the y-axis than the reference stepping  position, as in the human data. 30$^\circ$-crouch gaits are not necessarily the case, but the y values of more successful post-push steps are smaller than that of the reference position. This means that perturbation during the learning process allows learning policies that are more similar to the actual human balancing mechanism. The significant fatigue experienced by the human participants during crouch walking is not modeled in our simulation model, which might result in the slightly different tendency of post-push steps  for 30$^\circ$-crouch gaits.

% This observation seems contradictory to the previous study~\cite{lee2015push}, which reported that maximum detour distances are smaller for later-swing pushes with DDC. It is because the swing foot

% \color{red}
% What's the difference between the foot placement of normal walking and 30$^\circ$-crouch gait?
% At the early swing phase, 
% \color{black}

% \color{red} In the previous analysis \cite{lee2015push}, it is proved statistically that the later push timing, the shorter detour distance. They interpreted that when the external push occurs in late-swing phase, it is easy to put down the foot to enter the double stance phase quickly.
% In the view of foot placement, the later the push timing, the less time the character can step in the appropriate location.
% % is more resilient in Group 1 data in terms of the detour distance. When the external push occurs in late-swing phase, it is easy to put down the foot to enter the double stance phase quickly. 
% \color{black}

The plots in Figure~\ref{fig:foot_placement} depict the correlation between post-push foot placements and push magnitude/timing. DRL-A* learned its balance strategies based on foot placements, which are strongly correlated with how strong the disturbance is and when it occurs. DRL-A* is more robust than DRL-A at all push magnitudes and timings. DRL-A* adjusts its post-push foothold not only in the push (lateral) direction but also in the moving direction to better respond to the pushes.
We also observed the clear correlation of the number of detour steps with push magnitude. As push magnitude increases, the character needs one step ({\em Group 1} marked in blue) to three steps ({\em Group 2} - {\em Group 1} marked in green) to recover balance after the push.  
% The deep policies use one step to recovery the balance under the small disturbances. However, when the force is stronger, it use more steps for balance.  

\begin{figure}
\begin{subfigure}{.235\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/foot_placement_x_3d_fixed_length_speed_timing_3depth_adaptive_normal_nopush_small.pdf}  
  \caption{DRL-A (Pushing direction)}
  \label{fig:foot_placement_nopush_x}
\end{subfigure}
\begin{subfigure}{.235\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/foot_placement_y_3d_fixed_length_speed_timing_3depth_adaptive_normal_nopush_small_4sca.pdf}  
  \caption{DRL-A (Walking direction)}
  \label{fig:foot_placement_nopush_y}
\end{subfigure}
\vskip\baselineskip
\begin{subfigure}{.235\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/foot_placement_x_3d_fixed_length_speed_timing_3depth_adaptive_normal_push_small.pdf}  
  \caption{DRL-A* (Pushing direction)}
  \label{fig:foot_placement_push_x}
\end{subfigure}
\begin{subfigure}{.235\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/foot_placement_y_3d_fixed_length_speed_timing_3depth_adaptive_normal_push_small_4sca.pdf}  
  \caption{DRL-A* (Walking direction)}
  \label{fig:foot_placement_push_y}
\end{subfigure}
\caption{Foot placement plots at four push timings (13\%, 34\%, 55\%, 67\%). Green diamond indicates undisturbed reference step position. }
\label{fig:foot_placement}
\end{figure}




% \subsection{Energy Expenditure}

% \begin{figure}
%   \includegraphics[width=\columnwidth]{figures/cot2_plot.pdf}
%   \caption{Cost of transport.}
%   \label{fig:cot_plot}
% \end{figure}

% The relationship between gait speed and energy consumption has been previously studied in physiology \cite{snaterse2011distinct, ralston1958energy, anderson2001dynamic}. Humans supposedly choose a preferred walking speed that minimizes energy expenditure. The optimal speed reported so far ranges from 1.05 meter/sec~\cite{snaterse2011distinct} to 1.34 meter/sec~\cite{anderson2001dynamic}. Lee et al.~\shortcite{lee2015push} reported that the optimal speeds of simulated normal walking and 30$^\circ$-crouch walking are 1.0 meter/sec and 0.8 meter/sec, respectively, which are slower than previously reported values (see Figure~\ref{fig:cot_plot}).

% We conducted similar experiments to measure the optimal speed of normal and 30$^\circ$-crouch walking with DRL-B*. Cost of transport (COT), or energy expenditure per unit distance is a measure of how efficiently a human, an animal or vehicle has moved. The COT is defined as the energy used to move the body a unit of distance.
% \begin{equation}
%     COT = \frac{E}{mgd} = \frac{1}{mgd} \int \sum_{j} \|\tau_{j}\| \|\omega_{j}\| dt,
% \end{equation}
% where $m$ is the body mass, $g$ is gravitational acceleration, $d$ is a travel distance, $\tau_{j}$ and $\omega_{j}$ are the torque and angular velocity at joint $j$. Note that COT is dimensionless. In our experiments, the COT of normal and 30$^\circ$-crouch walking have optimal speeds at 1.29 meter/sec and 1.09 meter/sec, respectively, which are closer to previously reported values. It is also noticeable in the figure that DRL policies are more energy-efficient than DDC when they are learned from the same data set. 

% Figure~\ref{fig:cot_plot} and Table~\ref{fig:Sampling_success_rate} show a trade-off between stability and energy-efficiency. Normal walking is more energy-efficient than crouch walking because the straight leg in the stance phase supports the body weight with little torque at the knee joint. Crouch walking achieves improved stability and resilience against disturbances at the cost of extra energy consumption.


\subsection{Application: Interactive Control}

In an interactive control problem, it is critical to process the user input on-the-fly. A sudden change of the reference motion during the simulation can act as an impulse in the system. 
Since the gait-conditioned policies learn from diverse walking motions under disturbances, a simulated character controlled by these policies is robust to the change of input motions, and thus can transit from a gait pattern to another smoothly without any additional technique such as motion blending.


We demonstrate an interactive control to show the robustness of our gait-conditioned policies (Figure~\ref{fig:interactive_control}). In this example, we compare the four deep control policies: DRL-A*, DRL-B*, DRL-A, and DRL-B. Each character is controlled by a single control policy, and the reference motion is changed whenever the user input consisting of walking speed, stride length, and crouch angle is given. Despite diverse types of sabotaging with the obstacle, push forces, and repeated changes of input motion, the character controlled by DRL-A* survives alone to the last. Please refer the
supplemental video at (05:24). 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/interactive_control_figure}
    \caption{Interactive control. By using a single gait-conditioned policy, we can simulate a sequence of the biped walking motions that span a wide range of walking speeds, stride lengths, and crouch angles as well as the external pushes.}
    \label{fig:interactive_control}
\end{figure}

% are first crouched on-demand from 0 degrees to 60 degrees in order to go low, and then 
% While walking, the left and right alternating external perturbation are applied, and the magnitude of external forces are 50N, 100N, 150N, and 200N, respectively.
% In this example, all four characters walk with crouch from 0 to 60 degrees, passing through obstacles, but DRL-A and DRL-B could not withstand 100N of external shocks and fell.
% The DRL-A* and DRL-B* withstood up to 150N of external force, while the DRL-B * failed to withstand 200N of shock at a fast pace.


%Although the exact COT can not be calculated by our model because joint torque is the result of agonist and antagonist muscles working together and our model does not include any muscles, we still can estimate the tendency of COT value for our DRL controller with various speed. We calculate the COT as follows:


%----------------------------------------------------%






% \begin{table}
% \resizebox{\columnwidth}{!}
% {
% \begin{tabular}{lcccccc}
% \toprule
%                     %   &                     &   with Push    &               &                       & without Push  &               \\ 
%                       &     DRL-base        &       RL-BF    &  DRL-AD      &      DRL-base*        &   DRL-BF*     &  DRL-AD*      \\ \midrule
% Normal                &                     &       33.8     &   50.7       &                       &   26.0        &               \\ \hline
% Crouch $20\,^{\circ}$ &                     &       54.6     &   78.8       &                       &   22.1        &               \\ \hline
% Crouch $30\,^{\circ}$ &                     &       53.5     &   71.9       &                       &   11.1        &               \\ \hline
% Crouch $60\,^{\circ}$ &                     &       22.2     &   47.8       &                       &   9.4         &               \\ \bottomrule
% \end{tabular}
% }
% \bigskip\centering
% \caption{Experiment success rate (\%) of each control policies. 100N constant force and fixed push timing (34\%) are used for the experiment. Superscript * denotes control policies training without push. \color{red} Three layers-training version (for eliminating each crouch)}
% \label{tab:all_motion_success_rate}
% \end{table}


% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \footnotesize
% \begin{tabular}{|c|c|l|ll}
% \cline{1-3}
% \multicolumn{1}{|l|}{}                                                                            & \begin{tabular}[c]{@{}c@{}}Level of \\ Crouch\end{tabular} & \multicolumn{1}{c|}{Linear Mixed Models}                    &  &  \\ \cline{1-3}
% \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Human\\ Participants\end{tabular}}                     
%             & Normal         & $\alpha_{d}$ = 236.86 + 0.1898$\alpha_{f}$ - 0.02969$\alpha_{s}$ - 0.9951$\alpha_{t}$ + 69.2396 &  &  \\
% \cline{2-3} & $20\,^{\circ}$ & $\alpha_{d}$ = 236.86 + 0.1898$\alpha_{f}$ - 0.02969$\alpha_{s}$ - 0.9951$\alpha_{t}$ + 13.1796 &  &  \\ \cline{2-3} & $30\,^{\circ}$ & $\alpha_{d}$ = 236.86 + 0.1898$\alpha_{f}$ - 0.02969$\alpha_{s}$ - 0.9951$\alpha_{t}$ − 5.8181  &  &  \\ \cline{2-3} & $60\,^{\circ}$ & $\alpha_{d}$ = 236.86 + 0.1898$\alpha_{f}$ - 0.02969$\alpha_{s}$ - 0.9951$\alpha_{t}$           &  &  \\ \cline{1-3}
% \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Simulation\\ using\\ Feedback\\ Controller\end{tabular}} 
%             & Normal         & $\alpha_{d}$ = 247.5 + 0.4645$\alpha_{f}$ - 0.06404$\alpha_{s}$ - 1.8498$\alpha_{t}$ + 58.8934  &  &  \\
% \cline{2-3} & $20\,^{\circ}$ & $\alpha_{d}$ = 247.5 + 0.4645$\alpha_{f}$ - 0.06404$\alpha_{s}$ - 1.8498$\alpha_{t}$ + 36, 7256 &  &  \\ \cline{2-3} & $30\,^{\circ}$ & $\alpha_{d}$ = 247.5 + 0.4645$\alpha_{f}$ - 0.06404$\alpha_{s}$ - 1.8498$\alpha_{t}$ + 27.0606  &  &  \\ \cline{2-3} & $60\,^{\circ}$ & $\alpha_{d}$ = 247.5 + 0.4645$\alpha_{f}$ - 0.06404$\alpha_{s}$ - 1.8498$\alpha_{t}$            &  &  \\ \cline{1-3}
% \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Simulation \\ using \\ DRL \\Controller\end{tabular}}    
% & Normal                       & \multicolumn{1}{c|}{results}                                &  &  \\ 
% \cline{2-3} & $20\,^{\circ}$   & \multicolumn{1}{c|}{results}                                &  &  \\ 
% \cline{2-3} & $30\,^{\circ}$   & \multicolumn{1}{c|}{results}                                &  &  \\ 
% \cline{2-3} & $60\,^{\circ}$   & \multicolumn{1}{c|}{results}                                &  &  \\ 
% \cline{1-3}
% \end{tabular}
% \vspace*{5mm}
% \caption{\color{red} Test table for LMM. $\alpha_{d}$, $\alpha_{f}$, $\alpha_{s}$, and $\alpha_{t}$ indicate detour distance, push force, walking speed, and push timing, respectively.   \color{black}}
% \label{table:lmm1}
% \end{table}

% 하드웨어 스펙, RL training 시간 얼마나 걸렸는지.
% We used Intel® Core™ i9-9900K CPU @ 3.60GHz (8 cores) for training. Training takes a day for the baseline policies, and less than two days for the parameterized policies.
% The neural network for all DRL controllers consist of two fully connected layers with 256 nodes.
% Update for the neural network takes place when 2048 tuples collected with 128 batch size.
% % varies from 10 hours to two days according to the character model. 
% % Note that we used data normalized with respect to the character model's height and weight to exclude the effect by the character's structural factors.
% % 측정데이터들은 캐릭터 모델의 height and weight 로 normalize해서 사용.
% After training controllers with given conditions, push recovery experiment is conducted. 
% Previous research \cite{lee2015push} found out the decisive factors (level of crouch, walking speed, magnitude/timing of push) for the detour distance among 31 possible gait factors using linear mixed model (LMM).
% For the data earned from the computer simulation using DRL controller, we did statistical analysis for studying the effectiveness of each gait actor. We use R (version 3.6.1) for the statistical analysis.  
% % 이전 연구에서는 the linear mixed model (LMM)을 사용하여 31가지의 possible factors들 중에서 detour distance와 관련된 중요한 것들 (level of crouch, walking speed, magnitude/timing of push)을 골라냈다. 우리는 그 factor들에 대하여 statistical analysis를 진행하였다. 
% % 우리의 default setting은 조인트토크모델로, 모든 것을 다 control parameter로 넣고 push도 트레이닝하여 얻어낸 controller이다.
% % The numbers of experimental data used for each controller are described in the supplementary material.
% % 각 컨트롤러마다 사용한 실험 데이터의 개수는  supplementary material에 기재하겠다.
% % 캐릭터 모델이나 control parameter, sampling method를 바꿔가며 한 실험들에 대한 자세한 data 개수는 supplementary material에 기재하겠다.

% In the following section, we abbreviate the data driven controller proposed by the previous research \cite{lee2010data} as DDC.
% DRL-base, DRL-BF, and DRL-AD are abbreviations for DRL controller training baseline policies, DRL controller training parameterized policies using brute-force sampling, and DRL controller training parameterized policies using adaptive sampling, respectively.


% First, we analyze each control policy in perspective of the gait stability and expressiveness in section 5.1.
% In section 5.2, we compare our experimental data with human data and the previous simulation data in aspect of detour distance, and analysis is performed by group. Analysis of foot placement and cost of transport (COT) are followed in 5.3 and 5.4. 
% % 사람 데이터와 시뮬레이션 데이터와의 비교 분석을 위해 이전 연구와 같은 metric인 detour distance를 사용하였고, 이를 group별로 나누어 분석한 내용이 있다. 4.2에서는 foot placement 분석을 했다. 4.3에는 COT 분석을 하였다.
% % We deal with the difference between the results depending on the character models in 4.4. 
% Finally, in section 5.5, we evaluate each DRL trained controller which alters according to the various training conditions by analyzing the data with respect to the push recovery experiment success rate.
% 4.4 는 캐릭터 모델을 바꿔봤을 때의 분석을, 4.5에서는 training 에 variation을 줬을 때의 분석을 다루기로 하며, 여기서는 성공률을 기준으로 사용한다.

% \color{red}
% \begin{itemize}
%     \item 어떤 통계 기법을 어떻게 적용할지 논의 필요 
%     \item Bonferroni test (t-value, p -value)
% \end{itemize}
% \color{black}




% \subsection{Policy Analysis} 

% We introduce two different policies, baseline policies and parameterized policies.
% Each baseline policy is able to handle only one reference motion, while our parameterized policies can control various walking motions that have diverse speeds and stride lengths (Fig. ~\ref{fig:param_all}). 
% In terms of stability, however, which policies achieve superiority between the two policies?
% In order to compare the stability between two policies, we first selected nine pairs of walking speed and stride length on crouch $30\,^{\circ}$ motion, whose values are from mean -1 standard deviation to mean +2 standard deviation in human experiment data.
% Seven controllers were trained to obtain baseline policies for each speed-stride pair.
% % For the parameterized policies, we trained two kinds of controllers using brute-force parameter sampling and adaptive parameter sampling with the range of the mean $\pm2.5$ standard deviation.
% Then, we did push recovery experiments 1000 times for each control policy to measure the experiment success rate. When conducting the experiment, the magnitude and timing of push are randomly selected from the normal distribution of human data.
% %  baseline policies는 하나의 고정된 gait만을 컨트롤할 수 있는 반면, parameterized policies는 다양한 보폭과 보속을 가지는 walking motions들을 컨트롤할 수 있다 (Fig. ~\ref{fig:param_all}). 과연 안정성 측면에서 두 policies의 성능이 차이가 있을까? 이를 알아보기 위해서 실험을 했다. 우리는 보폭과 보속이 이루는 2차원 distribution을 9 단계로 discretize하였고 각각에 대해 baseline policies를 학습하였다. 그리고 uniform sampling과 adaptive sampling을 사용하여 two kinds of parameterized policies를 학습하였다.
% % 학습된 각각의 policies에 의해 제어되는 biped walking 시뮬레이션에 push recovery experiment를 천 번씩 진행한 후 성공률을 비교하였다. 실험 시 push force와 timing은 사람데이터의 normal distribution에서 sampling하였다. 

% Table ~\ref{fig:policy_comparison} shows the experiment with the success rate of each policies. 
% Success rate of DRL-BF is comparable with DRL-base for the motion having around the means of walking speed and stride length. However, as for slow motion with short stride length or fast motion with long stride length, DRL-BF controller could not withstand the external push for almost every force-timing pairs and fall down. It means that DRL controller trained with brute-force sampling can not cover all parameter region but only near the mean.
% Success rate of DRL-AD with the mean value is 79.8\% which is lower than other types of controllers, but highest at faster walking speeds (0.9 m/s and 1.01 m/s). Moreover, unlike DRL-BF which is robust only near the mean value, DRL-AD shows around 50\% success rate as for slower motion or faster motion. 
% Compared to DRL-base, both DRL-BF and DRL-AD are less stable, but DRL-AD is a method of training one network to cover broad range of walking motions as well as being equipped with acceptable stability over the entire range of gait parameters.

% DRL-AD의 경우, mean value 에서는 79.8\%로 성공률이 그리 높지는 않지만, 오히려 빠른 걸음들에서 높은 성공률을 보였다. 또한 mean value 랑 멀어지는 모션에 대해서도 50\% 안팎의 성공률을 보였다. 이는 DRL-BF의 경우 mean value 주변의 모션에서만 강건한 것과 사뭇 대조된다.  
% 물론 DRL-base와 비교해서는 DRL-BF와 DRL-AD 모두 안정성이 떨어지지만, DRL-AD는 하나의 네트워크만 트레이닝해서 여러 모션을 커버하며 안정성도 어느정도 확보하는 방법이라고 할 수 있다.
% adaptive sampling을 사용한 paramterized policy의 경우는 고르게 학습이 잘 되었다...?
% We claim that our parameterized policies with adaptive parameter sampling method, or DRL-AD have comparable stability with baseline policies, and also are effective to express wider range of motions in terms of walking speed and the step length.
% 우리는 parameterized policies는 안정성은 baseline 과 동등한데, 더 넓은 범위의 모션들을 커버할 수 있으므로, 표현력이 더 풍부하다라고 주장한다.

% \begin{table}
% \bigskip\centering
% \caption{Experiment success rate of each control policies. Mean parameter values are shown in gray.}
% %\resizebox{\columnwidth}{!}
% {
% \begin{tabular}{cccccccc}
% \toprule
%  Walking    &   Stride    &  DRL-base*  &   DRL-B*       &  DRL-A*      \\
% speed (m/s) &  length (m) &   (\%)      &   (\%)         &    (\%)      \\ \midrule
% %0.35        &	0.58       &   72.0      &                &              \\ 
% %0.46        &	0.67       &   90.9      &     fail       &    fail      \\ 
% 0.57        &	0.75      &   88.4      &      5.1       &    46.8     \\ 
% 0.68        &	0.83      &   88.2      &     85.9       &    55.6     \\ 
% \cellcolor[HTML]{D3D3D3}0.79&\cellcolor[HTML]{D3D3D3}0.92&   92.1      &     92.2       &    79.8     \\ 
% 0.90        &	1.00      &   87.6      &     86.5       &    97.5     \\ 
% 1.01        &	1.08      &   85.3      &     85.1       &    92.1     \\ 
% 1.12        &	1.17      &   97.3      &      0.0       &    71.9     \\ 
% 1.23        &	1.25      &   95.6      &      0.0       &    55.1     \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:policy_comparison}
% \end{table}

% \begin{table}
% \resizebox{\columnwidth}{!}
% {
% \begin{tabular}{cccccccc}
% \toprule
%  Walking    &   Stride    & DRL-base   &  DRL-base  &   DRL-BF   &  DRL-AD      \\
% speed (m/s) &  length (m) & nopush(\%) &   (\%)      &   (\%)    &    (\%)      \\ \midrule
% 0.35        &	0.58      &              &   72.0      &     fail  &    0.3       \\ \midrule
% 0.46        &	0.67      &              &   90.9      &     fail  &          \\ \midrule
% 0.57        &	0.75      &   10.7       &   88.4      &     1.8   &         \\ \midrule
% 0.68        &	0.83      &    5.4       &   88.2      &           &         \\ \midrule
% 0.79(Mean)  &0.92 (Mean)&    1.7       &   92.1      &           &         \\ \midrule
% 0.90        &	1.00      &    3.8       &   87.6      &           &         \\ \midrule
% 1.01        &	1.08      &    9.5       &   85.3      &           &         \\ \midrule
% 1.12        &	1.17      &    2.5       &   97.3      &           &         \\ \midrule
% 1.23        &	1.25      &              &   95.6      &           &         \\
% \bottomrule
% \end{tabular}
% }
% \bigskip\centering
% \caption{Experiment success rate of each control policies.}
% \label{tab:policy_comparison}
% \end{table}


%\subsection{Group Analysis} 

% Figure

% \begin{table}[ht]
% \resizebox{\columnwidth}{!}
% {
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{} & \multicolumn{4}{c|}{Group1}       & \multicolumn{4}{c|}{Group2}       \\ \cline{2-9} 
%                   & Normal & Crouch20  & Crouch30 & Crouch60 & Normal & Crouch20 & Crouch30 & Crouch60 \\ \hline
% success rate (\%) & 4.53   &        &        &  8.24  & 35.62  &  50.07 & 56.86  & 34.83  \\ \hline
% Min. force        & 78.55  &        &        & 62.70  & 78.55  &        &        &  -61.97  \\ \hline
% Max. force        & 265.56 &        &        & 282.36 & 318.30 &        &        &  -328.12 \\ \hline
% \end{tabular}
% }
% \caption{Experiment success rate when using the DRL controller.}
% \label{tab:distance_table}
% \end{table}


% 이전 연구에서 push test 후에 recovery step 측정해보니 one and three steps이 가장 많았다. DRL controller를 사용하여 시뮬레이션한 gait에 push recovery를 해놓고 성공한 실험들을 보니, 거의 대부분이 three steps 안에 recovery했다.
% We conducted push recovery experiments using the controllers training with DRL, examined the success data. 

% 실험 데이터에서 push recovery에 성공한 경우에 detour step은 세번 이하였다.
% The number of detour steps needed after pushing came out within three on successful experimental data, which is consistent with previous study. We examine the data by group. 
% 두 그룹으로 나눠서 분석해보기로 하였다.
% one step만에 regaining balance한 그룹을 group1, results regaining balance within three steps are group2 same as the previous research and 결과를 분석하였다.
% The numbers of experiment data of human and DRL simulation for the Group 1 are 228, 3727, respectively. The Group 2 data are results one recovered the balance within three steps. We used 450 human data, and 17735 DRL simulation data for the Group 2.
% In the case of successful push recovery for DRL simulation in experiment data, the detour step was mostly equal or less than three.
% Group 1 data are the results of taking one step to balance after a person or character is pushed.
% The numbers of experiment data of human, simulation, and DRL simulation for the Group 1 are 228, 3858, 3727, respectively.
% The Group 2 data are results one recovered the balance within three steps.
% We used 450 human data, 13707 simulation data, and 17735 DRL simulation data for the Group 2.

% The tendency that all the crouch gaits are more stable than normal gait is similar as the previous results (Fig. ~\ref{fig:distance_box_plot_each}).
% In our results, all motions have similar mean detour distance with human data, but have smaller standard deviations.
% When compared to the results of the previous feedback controller, the detour distance of DRL controller was lower.
% Overall, DRL controller is stable as human.
% 사람과 비슷한 수준으로 외부힘에 대해 안정적으로 반응한다고 할 수 있다. 또한, 이전 feedback controller보다 detour distance가 더 낮게 나오는 것을 보면 이전 컨트롤러보다 더 안정적이라고 말할 수 있다. 

% In our experimental results, crouch $60\,^{\circ}$ has the lowest detour distance than others. 
% Because we trained optimal controllers specifically for each level of crouch robust against the push force. 
% crouch 60도의 distance가 낮게 나오는 이유는 crouch 60도 모션에 대해서 외부 힘을 트레이닝했기 때문에, 학습이 잘 되어서이다. 
% 사람은 60도 자세를 유지하려면 근력이 많이 들고,자세 유지 자체가 힘들어서 밸런싱이 쉽게 깨질 우려가 있다. 
% Surprisingly, in group 1 and group 2, 
% normal gait and $20\,^{\circ}$ crouch gait have shorter detour distance than human data, which means more stable. $30\,^{\circ}$ crouch gait and $60\,^{\circ}$ crouch gait are less stable than humans but more stable than sim1.

% \newcolumntype{s}{>{\columncolor[HTML]{AAACED}} p{3cm}}
 
% \arrayrulecolor[HTML]{DB5800}

% \subsection{Comparison to Previous Feedback Rule Controller}

% 이전 컨트롤러 실험 결과와 비교.
% ys.
% \begin{itemize}
%     \item 기존 논문의 분석과 동일한 방식으로 분석하여 DRL의 경향성도 동일한지 분석 (group 1과 group 2)
%     \item 기존 논문의 data driven controller와 DRL controller의 경향성 및 성능의 비교 분석  (group 2)
%     \item DRL controller variant 간의 비교 분석 (황필이가 리스트업한 항목들). 물론 이중 하나 혹은 2~3개의 학습된 제어 정책을 가지고 1), 2)의 분석을 수행하긴 해야겠지.
% \end{itemize}

% We did type 3 test for the detour distance as a fixed effect. For both groups, all factors except the timing of push are significant (p < 0.05) in DRL simulation results (Table ~\ref{table:lmm1}). 
% In the previous study, the less the detour distance, the later push timing in Group 1, so later push timing is more stable. While in our results, push timing has no significance with detour distance.
% swing phase가 찰나의 순간이고, 미는 순간부터 0.2초 동안 미는 실험에서는, 늦게 밀면 stance phase와 가깝거나 겹치기 때문에 결국 실패 케이스가 된다. 결국 early timing에 push한 결과들만 성공 케이스로 분석되었다. 
% 이는 DRL controller가 push timing과 상관없는 적절한 foot placement strategy를 학습했다고 해석 가능하다. 
%It can be interpreted that the DRL controller has learned an appropriate foot placement strategy that is independent of push timing.
% Group1이나 Group 2 모두에서 Timing of push를 제외하고 모든 factors들에 대해 significant한 결과 (p < 0.005)가 나왔다. 

% \color{red}
% Group1과 Group2의 차이가 별반 나타나지 않는데, group analysis라고 하는 게 의미가 있는가...? 그냥 human data와 DRL의 비교분석 섹션으로 해야 하는가?
% \color{black}


% \begin{table}
% \resizebox{\columnwidth}{!}
% {
% \begin{tabular}{|c|c|c|c|c|c|cc|c|c|}
% \hline
% \multicolumn{2}{|c|}{\multirow{3}{*}{}} & \multicolumn{8}{c|}{Type 3 Tests for fixed effects}                                                                                               \\ \cline{3-10} 
% \multicolumn{2}{|c|}{}                  & \multicolumn{2}{c|}{Level of Crouch} & \multicolumn{2}{c|}{Push Magnitude} & \multicolumn{2}{c}{Walking Speed} & \multicolumn{2}{c|}{Push Timing} \\ \cline{3-10}
% \multicolumn{2}{|c|}{}   & $F_{c}$  & \multicolumn{1}{c|}{$p_{c}$}   & $F_{f}$  & \multicolumn{1}{c|}{$p_{f}$} & \multicolumn{1}{c|}{$F_{s}$} & \multicolumn{1}{c|}{$p_{s}$} & \multicolumn{1}{c|}{$F_{t}$} & \multicolumn{1}{c|}{$p_{t}$} \\ \hline\hline
% % Group1
% \multirow{3}{*}{Group 1}    & Human     & \cellcolor[HTML]{D3D3D3}17.49 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3} 13.42 & \cellcolor[HTML]{D3D3D3} 0.0003 & 2.68 & 0.1098 & \cellcolor[HTML]{D3D3D3} 14.35 & \cellcolor[HTML]{D3D3D3} <.0001   \\ \cline{2-10} 
%                             & DDC       & \cellcolor[HTML]{D3D3D3}{30.06} & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}17546 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}106.56 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}463.41 & \cellcolor[HTML]{D3D3D3}<.0001   \\ \cline{2-10} 
%                             & DRL-B*     & \cellcolor[HTML]{D3D3D3}612.7666 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}751.5370 & \cellcolor[HTML]{D3D3D3} <.0001 & \cellcolor[HTML]{D3D3D3}80.1890 & \cellcolor[HTML]{D3D3D3}<.0001 & 1.1668 & 0.2805  \\ \hline\hline
%                             % Group2                       
% \multirow{3}{*}{Group 2}    & Human    & \cellcolor[HTML]{D3D3D3}8.35 & \cellcolor[HTML]{D3D3D3}<.0001 & 0.01 & 0.9297 & 0.03 & 0.8578 & \cellcolor[HTML]{D3D3D3}3.94 & \cellcolor[HTML]{D3D3D3}0.0479  \\ \cline{2-10} 
%                             & DDC      & \cellcolor[HTML]{D3D3D3}{88.34} & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}19103 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}371 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}225.79 & \cellcolor[HTML]{D3D3D3}<.0001 \\ \cline{2-10} 
%                             & DRL-B*    & \cellcolor[HTML]{D3D3D3}4433.249 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}8204.248 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}1038.339 & \cellcolor[HTML]{D3D3D3}<.0001 &  0.258 & 0.6115              \\ \hline
% \end{tabular}
% }
% \vspace*{5mm}
% \caption{Type 3 tests for fixed effects (level of crouch, walking speed, magnitude/timing of push). We colored significant values ($p < 0.05$) as gray cells.}
% \label{table:lmm1}
% \end{table}


% \begin{table}
% \centering
% % \footnotesize
% \resizebox{\columnwidth}{!}
% {\begin{tabular}{|c|l|c|l|c|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{}  & \multicolumn{8}{c|}{Type 3 Tests for Fixed effects}  \\ \cline{3-10}  & \multicolumn{2}{c|}{Level of Crouch} & \multicolumn{2}{c|}{Push Magnitude}  & \multicolumn{2}{c|}{Walking Speed}  & \multicolumn{2}{c|}{Push Timing}  \\ \cline{2-9} 
%   & $F_{c}$  & \multicolumn{1}{c|}{$p_{c}$}   & $F_{f}$  & \multicolumn{1}{c|}{$p_{f}$} & \multicolumn{1}{c|}{$F_{s}$} & \multicolumn{1}{c|}{$p_{s}$} & \multicolumn{1}{c|}{$F_{t}$} & \multicolumn{1}{c|}{$p_{t}$} \\ \hline\hline
%   % Group1
%   \multicolumn{1}{|c|}
%   {\begin{tabular}[c]{@{}c@{}}Human\end{tabular}}   & \cellcolor[HTML]{D3D3D3}17.49 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3} 13.42 & \cellcolor[HTML]{D3D3D3} 0.0003 & 2.68 & 0.1098 & \cellcolor[HTML]{D3D3D3} 14.35 & \cellcolor[HTML]{D3D3D3} <.0001 \\ \hline \multicolumn{1}{|c|}
% {\begin{tabular}[c]{@{}c@{}}DDC\end{tabular}} & \cellcolor[HTML]{D3D3D3}{30.06} & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}17546 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}106.56 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}463.41 & \cellcolor[HTML]{D3D3D3}<.0001 \\ \hline
% \multicolumn{1}{|c|}
% {\begin{tabular}[c]{@{}c@{}}$DRL-B^*$\end{tabular}} & \cellcolor[HTML]{D3D3D3}612.7666 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}751.5370 & \cellcolor[HTML]{D3D3D3} <.0001 & \cellcolor[HTML]{D3D3D3}80.1890 & \cellcolor[HTML]{D3D3D3}<.0001 & 1.1668 & 0.2805 \\ \hline\hline
% % Group2
% \multicolumn{1}{|c|}
% {\begin{tabular}[c]{@{}c@{}}Human\end{tabular}} & \cellcolor[HTML]{D3D3D3}8.35 & \cellcolor[HTML]{D3D3D3}<.0001 & 0.01 & 0.9297 & 0.03 & 0.8578 & \cellcolor[HTML]{D3D3D3}3.94 & \cellcolor[HTML]{D3D3D3}0.0479 \\ \hline \multicolumn{1}{|c|}
% {\begin{tabular}[c]{@{}c@{}}DDC\end{tabular}} & \cellcolor[HTML]{D3D3D3}{88.34} & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}19103 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}371 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}225.79 & \cellcolor[HTML]{D3D3D3}<.0001 \\ \hline \multicolumn{1}{|c|}
% {\begin{tabular}[c]{@{}c@{}}$DRL-B^*$\end{tabular}} & \cellcolor[HTML]{D3D3D3}4433.249 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}8204.248 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}1038.339 & \cellcolor[HTML]{D3D3D3}<.0001 &  0.258 & 0.6115 \\ \hline
% % \hline
% % all
% % \multicolumn{1}{|c|}
% % {\begin{tabular}[c]{@{}c@{}}$Human^{(all)}$\end{tabular}}   & \cellcolor[HTML]{D3D3D3}6.33833 & \cellcolor[HTML]{D3D3D3} 0.0121 & 0.00021 & 0.9884 & 2.95934 & 0.0859 & \cellcolor[HTML]{D3D3D3}9.29231 & \cellcolor[HTML]{D3D3D3}0.0024 \\ \hline \multicolumn{1}{|c|}
% % {\begin{tabular}[c]{@{}c@{}}$Sim1^{(all)}$\end{tabular}} & \cellcolor[HTML]{D3D3D3}{158.666} & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}19115.434 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}334.907 & \cellcolor[HTML]{D3D3D3}<.0001  & \cellcolor[HTML]{D3D3D3}223.443 & \cellcolor[HTML]{D3D3D3}<.0001 \\ \hline\multicolumn{1}{|c|}
% % {\begin{tabular}[c]{@{}c@{}}$Sim2^{(all)}$\end{tabular}} & \cellcolor[HTML]{D3D3D3}31.59578 & \cellcolor[HTML]{D3D3D3}<.0001  & \cellcolor[HTML]{D3D3D3}147.95901 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}28.30370 & \cellcolor[HTML]{D3D3D3}<.0001 & \cellcolor[HTML]{D3D3D3}54.73096 & \cellcolor[HTML]{D3D3D3}<.0001 \\ \hline
% \end{tabular}}
% \vspace*{5mm}
% \caption{Type 3 tests for fixed effects (level of crouch, walking speed, magnitude/timing of push). We colored significant values ($p < 0.05$) as gray cells.}
% \label{table:lmm1}
% \end{table}

% \begin{figure}[ht]
%   \includegraphics[width=\columnwidth]{figures/foot_placement_2d.pdf}
%   \includegraphics[width=\columnwidth]{figures/foot_placement_3d_com_vel_x.pdf}
%   \includegraphics[width=\columnwidth]{figures/foot_placement_3d_com_vel_y.pdf}
%   \caption{Each crouch (30도) + push+ uniform sampling 사용한 controller를 constant force (100N), fixed push timing으로 천 번 실험한 결과 데이터의 Foot placement. Blue dot means success case, and red dot means failure case. }
%   \label{fig:foot_placement}
% \end{figure}


% \begin{figure}[ht]
%   \includegraphics[width=\columnwidth]{figures/foot_placement_2d.pdf}
%   \includegraphics[width=\columnwidth]{figures/foot_placement_3d_com_vel_x.pdf}
%   \includegraphics[width=\columnwidth]{figures/foot_placement_3d_com_vel_y.pdf}
%   \caption{Each crouch (30도) + push+ uniform sampling 사용한 controller를 constant force (100N), fixed push timing으로 천 번 실험한 결과 데이터의 Foot placement. Blue dot means success case, and red dot means failure case. }
%   \label{fig:foot_placement}
% \end{figure}

% \subsection{Foot Placement Analysis}

% \begin{figure*}
%     \begin{subfigure}{.3\textwidth}
%       \centering
%       % include second image
%       \includegraphics[width=\linewidth]{figures/human_foot_placement_2d_fixed_length_speed_zerofoot_origin_new.pdf}  
%       \caption{Human data}
%       \label{fig:foot_placement_human}
%     \end{subfigure}
%     % \vskip\baselineskip
%     \begin{subfigure}{.3\textwidth}
%       \centering
%       % include third image
%       \includegraphics[width=\linewidth]{figures/foot_placement_2d_fixed_length_speed_zerofoot_origin_new.pdf}  
%       \caption{Training with Push}
%       \label{fig:foot_placement_push}
%     \end{subfigure}
%     \begin{subfigure}{.3\textwidth}
%       \centering
%       % include fourth image
%       \includegraphics[width=\linewidth]{figures/NO_push_foot_placement_2d_fixed_length_speed_zerofoot_origin_new.pdf}  
%       \caption{Training without push}
%       \label{fig:foot_placement_nopush}
%     \end{subfigure}
%     \caption{Foot placement plot. Blue dot and red dot indicate success and failure case, respectively, and green diamond means the original foot placement when there exists no external perturbation. Relative location of the stance foot is the origin which is represented as a magenta diamond.}
%     \label{fig:foot_placement_fixed_speed_step_length}
% \end{figure*}


% It is known that deciding the foot landing location is important for balance. 
% While walking, when getting into the environment such as the bumpy terrain or icy ground, or unexpected external force is applied, human maintains the balance by stepping at the proper location.
% % In other words, if one can step to the proper position, then balance can be kept.
% % 그렇다면 발 내려놓는 위치를 성공적으로 결정하는데 결정적인 factor가 있고, 이를 찾아볼 수 있지 않을까?
% % 시뮬레이션 실험 데이터에서 발의 위치를 뽑아내어 여러 가지 factor들과 분석한 결과 다음와 같은 결과를 얻었다.
% % 밸런싱에 성공한 아이들과 그렇지 못한 아이들의 발 위치는 어떤 factor에 의하여 갈렸다.
% To figure out the tendency of the foot placement when the external push force is applied, we fixed other gait factors (walking speed, stride length, level of crouch) and let only the magnitude and timing of push be variables. 
% We conducted push recovery experiments using DRL-BF for crouch $30\,^{\circ}$.
% % 우리는 어떤 한 factor에 대한 영향력을 보기 위해서 다른 gait factor들을 고정시켜 놓고 push recovery experiments를 진행해보았다. 
% Fixed value is determined by the mean value of normal distribution of human data (Table \ref{tab:human_data_mean}).
% % except push magnitude. Note that we used one of the three constant values (50N, 100N, 150N) for magnitude of push.



% % 보폭과 보속을 바꿔가며 걷는 걸음에 대해서 미는 힘과 타이밍을 고정하고 실험해본 결과, 성공하는 실험의 foot placement가 어느정도 응집되게 나타났지만 뚜렷한 경향성은 보지 못했다 (Fig. \ref{fig:foot_placement_a}). 
% Fig. \ref{fig:foot_placement_fixed_speed_step_length} shows the foot placements of human data and data of two control policies, training with push/without push. For plotting human data (Fig. ~\ref{fig:foot_placement_human}), we used 22 crouch $30\,^{\circ}$ data of human subjects. 
% The foot placement of experimental results using push training (Fig. ~\ref{fig:foot_placement_push}) is consistent with human data (Fig. ~\ref{fig:foot_placement_human}) in aspect that it balances by stepping backward from the original stepping position.
% %  \ref{fig:foot_placement_human} . 보면 원래 발 디디는 위치보다 뒤 쪽으로 디디며 중심을 잡는다는 측면에서, It matches with the Fig. ~\ref{fig:foot_placement_push}.
% % 보폭과 보속을 고정하고, 미는 힘의 크기와 타이밍을 바꿔봤을 때는 (Fig. \ref{fig:foot_placement_fixed_speed_step_length})와 같이 더 확실히 응집되어 나타났다. 
% In Fig. ~\ref{fig:foot_placement_human}, it seems that human data has no clear tendency with respect to the groups. Note that human data is earned from the different individuals. Moreover, unlike the simulation data, it is impossible to collect the data subject to human under the situation controlling the variables like walking speed, stride length, magnitude/timing of the push. In other words, human data is unbalanced and sparse. For example, the push timings of human data are mostly distributed between 20\% and 50\%. 
% % 사람데이터는 여러 체중과 신장이 다른 subject들의 속도와 보폭이 고정되지 않은 데이터이다 보니 시뮬레이션 결과에 비해 데이터들이 응집되지 않아 경향성을 보기는 어렵다는 것을 감안해야 한다.
% % 사람 데이터가 original stepping position 근처에 많이 없는 이유는, 사람 대상으로 한 실험에서 오른발 스윙 시에 밀라고 했는데, 이 찰나의 순간에 밀다보니 아무래도 균일한 타이밍으로 밀기가 어려웠고, 대부분의 데이터가 push timing 인터벌 20\%\~50\% 사이에 push한 것들 뿐이기 때문이다.




% % The reason why the step widths of human data is narrower than the simulation is that human participants are instructed to walk following the line during the experiment.
% % 사람의 두 발의 간격이 시뮬레이션보다 좁은 이유는 실험 시에 사람이 밀릴 것을 예상했기 때문이다...?
% % \color{red}
% % 사람의 보행 간격 (step width)은 보통 5, 13cm 가 적당하다. 고 인터넷에 나오네...
% % 사람 데이터가 정상인 듯... 그러면 시뮬레이션 데이터는 왜케 넓은가?
% % (1) 사용한 모션 데이터 자체가 보행 간격 넓은 데이터이다. (2) 트레이닝 중에 보행 간격이 넓어지도록 학습되었다.
% % \color{black}
% The reason the step width of simulation data is wider than the human is that the reference motion data itself we used has wide step width.



% \subsection{Energy Expenditure}

% \begin{figure}
%   \includegraphics[width=\columnwidth]{figures/cot2_plot.pdf}
%   \caption{Cost of Transport (COT).}
%   \label{fig:cot_plot}
% \end{figure}

% There are several studies which explore the relationship between gait speed and energy consumption in physiology \cite{snaterse2011distinct, ralston1958energy, anderson2001dynamic}. The results shows that relation of walking speed and the energy consumption appeared parabola shape, and human tends to prefer to walk at the speed which minimizes the energy expenditure.
% % It is known that human walks at the preferred speed which minimizes the energy expenditure. 
% Cost of transport (COT) or energy expenditure per unit distance were used as measurement of human experiments. Optimal speed is reported that approximately 1.05m/s, 1.24m/s (74m/min), 1.34m/s (80m/min), respectively.
% We measured COT values from our simulation results where the walking speed is sampled from the normal distribution of human data.
% % In our set up, as for the joint-torque model, we measure COT values, and for the musculoskeletal model, we measure the metabolic energy expenditure. 메타볼릭 에너지는 muscle mass 정보가 없어서 구할 수 없음...
% Fig. ~\ref{fig:cot_plot} conformed that the tendency of the parabolic shape is same as humans. In both cases (DRL-A* and DRL-B*), normal walking has the optimal speed at 1.3 meter/second approximately, while crouch $30\,^{\circ}$ has slower peak speed. Also, the COT of normal walking is lower than the COT of crouch data, as we expected.
% Moreover, the optimal speed from COT results obtained by DRL-BF is closer to that of human experimental results.
% 이전 시뮬레이션 데이터는 normal의 optimal speed가 1.0m/s 이었는데, drl controller의 결과가 사람의 optimal speed 절대치와 더 가깝다.
%while all other crouch motions are slower than normal gait and consume more energy.


% Snaterse et al \cite{snaterse2011distinct} 
% Ralston et al \cite{ralston1958energy} identified the relationship between speed and energy when human walking. To mearsu
% DRL 컨트롤러로 나오는 모션의 Cost of Transport (COT)가 파라볼릭한 형태가 나오고 (Fig. ~\ref{fig:cot_plot}), 사람의 range (1.05m/s ~1.4 m/s)와 비슷하게 나오면 의미가 있으려나... 
% 실제 사람의 walking을 가지고 속도와 에너지의 관계를 정립한 논문이 있다 \cite{anderson2001dynamic}. 이 논문에서는 metabolic energy / Distance traveled [calories/(m x kg)] = 80m/minute =1.34m/s 라고 했는뎅.... muscle model의 에너지랑 비교 가능할 듯. 

% \subsection{Character Model Analysis}

% Here DRL을 통해서 컨트롤할 때 신체 모델이 어떤 영향을 끼치는지에 대해 분석해보았다. 
% 실제 사람은 뇌에서부터 전기신호를 받아서 근육을 수축 또는 이완시키며 이런 근육의 합력이 주변의 joint들에게 torque를 발생시켜서 움직인다. 그러나 간단한 신체 모델링이 제어가 편하기 때문에, 모터로 이루어진 로봇과 같은 joint torque body model을 사용하여 이족보행을 제어하는 연구가 많았다. 최근 들어서 실제 사람과 흡사한 신체 모델링을 하는 연구들이 많이 진행되었고, 좋은 결과들을 보여주었다. 
% We can train with different models which are actuated different way: muscle actuated and joint-torque actuated. 
% As expected, musculoskeletal model shows similar with human data than joint torque model.
% % Also, to evaluate the effectiveness of the complex foot model, we use multi-segment foot model for training the DRL controller. 
% \color{red}
% character model을 바꿔서 실험했을 때 어떤 결과가 나오는지, 다른 점을 어떤식으로 보여줄지... 고민...

% 일단은, with push trained controller 의 성공률은 조인트 토크모델의 성공률보다 좋게 나왔으면 하고, 놀랍게도! 
% without push trained controller의 경우 조인트 토크 모델보다 월등하게 좋았다는 점을 밀자. 이게 왜 그러냐면, 근육간의 코엑티베이션 작용 때문에 충격 흡수? 를 할 수 있어서 외부 힘에 더 잘 버틸 수 있다는 식으로 설명하는거다.
% \color{black}


% 각각의 variant의 의미를 기술하면 좋을 것 같다.
% 사람이 어떤 식으로 걷는지를 매치해서 생각해보는 거다.
% 따라서 결론적으로 이런 variation들에 대해서 각각의 biped controller를 학습해보고, 과연 결과가 어떤지를 살펴보겠다.
% 예상하기로는 adaptive, each crouch가 더 좋다, 또는 사람과 더 가깝다?. 그리고 with/without push 는 사람에게 둘 다 가능한 시나리오인데 뭐 당연히 push를 학습한 controller가 더 강건하겠다... 이런식으로?  

% 이런 variation들에 대해서 각각의 biped controller를 학습해보고, 과연 결과가 어떤지를 살펴보겠다.

% \paragraph{Training with one motion / several motion. }

% Data driven controller need reference motions to mimic. 
% Researches about controlling diverse motions using one network have been conducted \cite{2018-TOG-deepMimic, Park:2019}.
% % 하나의 DRL 컨트롤러로 여러 모션을 학습하려는 연구들이 진행되어 왔다 \cite{2018-TOG-deepMimic, Park:2019}. 
% % 그러나 안정성 측면에서 하나의 모션만을 tracking하는 것, 여러가지 모션을 함께 학습하는 것, 둘 중에 어떤 학습 방법이 더 좋을까?
% In terms of stability, which controller can be more resistant to external perturbation, a controller trained for one reference motion or a controller trained for multiple motions?
% % 한 가지 레퍼런스 모션만 특정한 controller와 여러 가지 모션들을 커버할 수 있는 controller 중에 어떤 것이 더 외부 섭동에 대해 안정적일 수 있을까?
% % DRL controller와 같은 경우는 하나의 reference motion에 대해 학습한 경우와 여러 개의 모션을 가지고 학습하는 두 경우를 생각해볼 수 있다. 
% Among crucial gait factors, level of crouch is discrete factor (normal, crouch $20\,^{\circ}$, crouch $30\,^{\circ}$, crouch $60\,^{\circ}$ ). We consider that there are four motions according to the level of the crouch. We train controllers individually tracking for each crouch motion, a controller tracking for all crouch motions.
% % 이 크라우치 레벨에 따라 네 개의 모션이 있다고 생각하고, 이 모션을 각각을 트레이닝시킨 컨트롤러들과 모든 모션에 대해 트레이닝시킨 컨트롤러의 학습 및 비교가 가능하다.
% % 사람의 경우로 친다면, 어떤 동작을 학습하기 위해서 한 가지 동작만을 계속 연습한 사람과, 여러 가지 동작을 두루두루 연습한 사람을 비교하는 것이다.

% In case of training with push force, the success rates of the push recovery experiment of the controller for each motion are higher than those of the controller for multiple motions (Table ~\ref{tab:motion_success_rate}).   
% Consequently, we confirmed that training a control policies for each motion is more robust to the external perturbation.

% % 실험성공률로 보아 결론적으로 all level crouch 모션에 대해 학습시킨 컨트롤러보다 각각의 crouch level motion에 대해 학습시킨 컨트롤러가 more robust to the external perturbation (Table ~\ref{tab:motion_success_rate}).
% Interestingly, in case of training without push, the success rates of normal walking and crouch $20\,^{\circ}$ of the controller for multiple motions are higher. 
% It can be interpreted that some degree of flexibility is increased while learning about several motions, even in the situation where untrained external force is applied. 
% % 흥미로운 점은, nopush training의 경우에는 multiple motion을 학습한 것이 normal gait와 crouch 20도에 대해서는(com 이 높은 모션들) 성공률이 더 높았다. 여러 모션에 대해 학습하면서 하나의 모션에만 확실히 fit되어 학습되지는 못했지만 유연성이 증가하여 학습되지 않은 외부힘이 가해지는 상황에서도 어느정도 버텼다고 생각할 수 있겠다.
% % push를 학습하지 않은 경우, 각각의 모션에 대한 컨트롤러의 실험 성공률은 crouch level이 높아질 수록 성공률이 높아지고, multi motion controller는 크라우치 레벨이 높아질수록 성공률이 낮아졌다. 이는 crouch level이 높아질수록 com이 낮아져서 안정적이 되는 것 같다.

% % 따로 Each level of crouch motion을 학습한 컨트롤러의 push recovery experiment 성공률이 대체로 all crouch로 학습한 컨트롤러의 실험 성공률보다 높았다 (crouch 20도를 제외하고). 특히 crouch 60도에서 차이가 많이 났다. 성공률이 all crouch로 학습했을 때가 5.11\%로 현저히 낮았다 (Table ~\ref{tab:push_success_all}). 
% % % 그나마 성공한 tuple들의 push magnitude distribution을 plot해 봤을 때 mean force보다 낮은 약한 힘에서만 잘 버틴 것을 관찰할 수 있었다 (Fig. ~\ref{fig:param_allpush}). 
% % 따라서 push apply해서 학습을 했어도 all level crouch를 파라미터라이즈하여 학습했을 때는 모든 crouch motion이 외부 힘에 robust하게 버티도록 학습이 잘 되지는 않았다. 
% % push를 넣지 않았을 때는 all crouch나 each crouch나 실험 성공률이 매우 저조했으나, 그나마 each crouch로 학습한 컨트롤러의 성공률이 더 높게 나왔다.
% % 결론적으로 all level crouch 모션에 대해 학습시킨 컨트롤러보다 각각의 crouch level motion에 대해 학습시킨 컨트롤러가 more robust to the external perturbation. 


% % uniform parameter sampling과 push 넣어서 학습한 경우에 보면 어떤어떤 경향성을 보였다.

% % uniform parameter sampling과 push 넣어서 학습한 경우에 보면 각각의 모션을 학습한 경우가 모든 모션을 학습한 경우보다 성공률이 높았다 (Table ~\ref{tab:push_success_all_torque_drl_only_100N_type3_included}). 그러나 회색으로 표시한 경우에 보면 반대의 경향성이 나타났는데, 이는 큰 힘 (100N, 150N)에 대해서 crouch가 미약한 normal gait나 20도 crouch의 경우다. 이 경우는 push가 없이 학습한 경우임을 감안하고, 각각을 학습한 경우에는 외부 힘에 대해서 모션의 융통성? flexibility? 유도리? 바뀌는 능력?이 없어서 부러진거지. 버티지 못하고 넘어진 것이다. 그렇지만, 여러 모션에 대해 학습한 경우는 push 없이 학습했음에도 어느정도 유연함을 갖출 수 있어 저 경우에 버틸 수 있었다고 해석하였다.

% % 결론적으로 all level crouch 모션에 대해 학습시킨 컨트롤러보다 각각의 crouch level motion에 대해 학습시킨 컨트롤러가 more robust to the external perturbation (Table ~\ref{tab:motion_success_rate}). 


% \begin{table}
% \bigskip\centering
% \caption{Experiment success rate (\%).}
% \resizebox{\columnwidth}{!}
% {
% \begin{tabular}{lccccc}
% \toprule
%                       &         DRL-B*      &                &       DRL-B           &               \\ \midrule
%                       &     Multi-Motions   &    One Motion  &    Multi-Motions      &  One Motion   \\ \midrule
% Normal                &        33.8         &       62.5     &           26.0        &     2.6       \\ 
% Crouch $20\,^{\circ}$ &         54.6        &       66.7     &           22.1        &     12.4      \\ 
% Crouch $30\,^{\circ}$ &         53.5        &       72.0     &           11.1        &     31.3      \\ 
% Crouch $60\,^{\circ}$ &         22.2        &       53.8     &           9.4         &     47.0      \\ 
% \bottomrule
% \end{tabular}
% }
% \label{tab:motion_success_rate}
% \end{table}


% \paragraph{Training with/without push.}

% % With push training은 사람이 밀릴 것을 예상하고 걷는 것을 학습한 것이고, without push는 사람이 외부힘을 예상하지 않고 걷는 모션을 학습한 것이다. 
% % DRL은 noise를 주면서 학습을 하기 때문에 어느 정도의 외부 섭동에 robust하다는 결과들이 많이 있다.
% Controllers trained with DRL can deal with the modest external perturbation because DRL takes trial-and-error approaches by given noise. 
% % 우리는 As we apply large push during walking, 
% However, depending on the presence of large amount of the external force during training process, the stability of the controller may change.
% We did experiments using two controllers, one trained with push force and the other trained without push force.


% A controller which is trained under the push force is more robust than that trained without push force (Table ~\ref{fig:Sampling_success_rate}). The success rate of the push-trained controller is especially high at crouch $20\,^{\circ}$ and crouch $30\,^{\circ}$. In experiment using a controller trained without push, the success rate is very low, but the higher the level of crouch, the higher the success rate. This can be interpreted as the lower the COM position, the higher the stability against external force.
% % 확실히 push를 넣고 트레이닝한 것이 외부 push에 대해서 robust했다 (Table ~\ref{tab:Push_success_rate}). 
% % push 없이 training한 컨트롤러로 실험한 결과, 실험 성공률이 매우 저조했다. 
% % with Push training의 실험 결과를 보면 crouch 20도와 crouch 30도의 성공률이 높았다. 
% % 반면에 without push training 실험 결과는, level of crouch가 높아질수록, 실험 성공률이 높았다. 이는 단순히 com 위치가 낮아질수록 외부힘에 대한 안정성이 높아졌다고 해석 가능하다.

% % 이전 논문에서 사람을 대상으로 한 push recovery 실험 데이터에서 보면 detour distance와 statistical analysis 두 가지 지표에서 모두 crouch 20도와 30도가 normal gait보다 더 안정적이라고 밝혀져 있다. 
% % DRL controller 실험을 push 넣고 했을 때와 안 넣고 했을 때의 성공률 경향성을 보면, 사람데이터는 push에 학습된 걸음걸이를 걷고 있다고 볼 수 있다. 그러니까 평소에 외부의 힘에 대비하면서 걷고 있다고 생각할 수 있다. 
% % push force를 학습하지 않은 controller와 학습한 controller 두 가지에 대하여 각각, 보속과 보폭을 고정한 채, 힘의 크기를 바꾸어보며 push recovery 실험을 진행하였다. 
% % 그리고 이 경우의 foot placement를 비교해 보았다 (Fig. ~\ref{fig:foot_placement_fixed_speed_step_length}). 
% Also, in both cases, we compare the foot placement (Fig. ~\ref{fig:foot_placement_fixed_speed_step_length}).
% The controller which is not trained for the external push force let a character's swing foot put forward than the original spot it would be, which make the character lose its balance to fall (Fig. ~\ref{fig:foot_placement_nopush}).  
% While, the push-trained controller which has learned the foot placement strategy makes a character step backward to maintain balance (Fig. ~\ref{fig:foot_placement_push}). 
% % No push trained controller의 경우는 대부분 swing foot을 앞으로 디디는 것이 실패의 요인이었고 (Fig. ~\ref{fig:foot_placement_nopush}), push trained controller의 경우는 swing foot을 앞으로 디디기 보다는, 뒤쪽으로 발을 디뎌서 밸런싱을 유지하는 것을 학습하였다 (Fig. ~\ref{fig:foot_placement_push}).
% % 결론적으로, 외부 힘에 대해서 밸런싱을 유지하기 위해서 foot placement가 중요한 factor라는 것을 확인할 수 있었다.



% In order to examine the foot placement in more detail, we analyze how the position of the foot tends to change as the force changes about four fixed push timings (13\%, 34\%, 55\%, 76\%) (Fig. ~\ref{fig:foot_placement}).
% % 더 자세한 분석을 위해서 고정된 네 개의 타이밍 (13\%, 34\%, 55\%, 76\%)에 대하여, 힘의 크기를 바꿔가며 실험해보고 plot해보았다 (Fig. ~\ref{fig:foot_placement}). 
% Note that in case of using no push training, we used push force distribution having smaller mean value (75N), because the simulated character cannot endure the force sampled from the original force distribution of human data.
% % No push의 경우, 사람 데이터의 평균힘으로 실험하면 다 실패하기 때문에, 분석을 위해서 적은 힘으로 밀어주었다. 

% % 보폭과 보속을 고정하고 미는 타이밍까지 고정해보니 (Fig. \ref{fig:foot_placement})와 같이 힘이 클 수록 못 버티는 것을 알 수 있었다. 

% Focusing on the heading direction (y) of the character, in the case of no push training, the swing foot was found to be in front of the original position (Fig. ~\ref{fig:foot_placement_nopush_y}). On the other hand, in the case of push training, it was confirmed that the foot was moved backwards than the original tread position (Fig. ~\ref{fig:foot_placement_push_y}).
% % 캐릭터의 진행방향 축에 초점을 맞춰 살펴보면, push training의 경우는 확실히 원래 디딜 위치보다 뒤쪽으로 발을 디디는 것을 확인하였다 (Fig. ~\ref{fig:foot_placement_push_y}). 반면에 no push training의 경우는 원래 발을 디딜 위치보다 앞쪽에 디디는 경향성을 확인했다 (Fig. ~\ref{fig:foot_placement_nopush_y}).

% On the direction of push, even a small external force in late swing phase (55\% and 76\%) can cause character to fall in both cases of the training with/without push. It is because the foot is about to touch the ground, and the character does not have enough time to change the foot position to be safe.
% For the case of training without push, the stronger the force, the farther the foot step position on the line (Fig. \ref{fig:foot_placement_nopush_x}).
% Interestingly, in the case of training with push, the foot step positions form parabola as the pushing force become stronger, especially when the push takes place in early swing phase (13\% and 34\%).
% % 미는 방향 축으로 살펴보면, push, no push 두 경우 모두, 늦은 swing phase (55\%, 76\%에서는 적은 힘으로 밀렸을 때도 실패하는 경우를 관찰 할 수 있었다.
% % 이는 늦은 swing phase에서는 발이 땅에 닿기 직전이기 때문에 발의 위치를 많이 변경할 수 없기 때문이다.
% % no push를 트레이닝의 경우는 힘이 증가하면 미는 방향으로 점점 발을 멀리 디디는 일직선 형태로 나온다 (Fig. \ref{fig:foot_placement_nopush_x}).
% % 흥미로운 점은, push 트레이닝한 경우에, early swing phase들 (13\%, 34\%)에서 힘이 증가할수록 미는 방향으로 그래프가 증가하는 게 아니라, parabolic한 형태가 나온다는 것이다 (Fig. \ref{fig:foot_placement_push_x}).
% When pushed with the modest force (up to 180 N) at the 13\% of push timing, the simulated character recovers balance using one step widening step width.
% However, the magnitude of the push force applied increases, the character uses three steps to recover balance (Fig. ~\ref{fig:group1group2_push}).
% We confirmed that the DRL controller learned to change the foot placement strategy based on the magnitude of the force as human does.
% Please, see the result video for detail.
% 13\% push timing으로 밀어준 경우, 어느 정도의 힘 (180N)까지는 힘이 커질수록 옆으로 발을 디뎌서 support region을 넓혀가면서 버티다가, 그 이상부터는 오히려 detour distance를 좁히면서 균형을 잡았다. 이는 balancing을 위해 step 수를 달리한 정책으로 설명할 수 있다. 힘이 커지만 one step만에 균형을 복구해낼 수 있다. 그러나 힘이 커지면 one step만에 균형을 복구가 어렵고, 그래서 three steps을 사용하여 균형을 잡는 정책으로 바뀌는 것이다. 즉, 힘이 커지면 foot placement 한 번 사용하던 정책을 세 번 사용하여 균형을 복구하는 정책으로 바꾼다는 것이다. 우리는 시뮬레이션 모션 결과로부터 이를 확인하였다 (Fig. ~\ref{fig:group1group2_push}). 
% 비디오를 참조해라.

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/group1_fig.pdf}
%     \includegraphics[width=\columnwidth]{figures/group2_fig.pdf}
%     \caption{DRL-A* learns strategies for balancing in one foot step for small external forces (100N) and two steps for large external forces (250N).
%     %\color{red} push training한 controller의 경우, 작은 힘 (100N)으로 밀릴 때는 one step만에(top), 큰 힘 (250N)으로 밀릴 때는 three steps을 사용하여 (bottom) 균형을 유지하는 정책을 러닝하였다.
%     }
%     \label{fig:group1group2_push}
% \end{figure}

% \color{red}
% 이는 push training controller가 foot placement strategy 말고 다른 balancing strategy를 학습했다고 추론할 수 있다. 그게 뭘까??? 상체나 팔을 미는 방향 쪽으로 기울인다던가 해서 COM 위치를 안정적으로 맞춘다던가?? 시뮬레이션 모션을 보면서 확인해봐야겠음!!
% 모션 확인해보니, 큰 힘에서는 three steps 만에 균형 recovery했다. 그래서 두 개의 swing foot에 대한 foot placement를 배운 듯하다... 
% \color{black}
% 보폭과 보속을 고정하고 미는 힘을 고정시켜서 실험을 했을 때는, 미는 타이밍이 거의 swing phase가 끝나가는 시점, 그러니까 heel strike (double stance)에 다다랐을 때 실패하는 것으로 나왔다 (Fig. \ref{fig:foot_placement_d}).  



% foot placement를 잘 하면, projection된 COM 위치가 support region 안에 오도록 한다는 말인데, no push의 경우는 이걸 잘 못한거지.. 

% all crouch motions이 다 10\% 미만이었다. crouch 60와 crouch 30도가 그나마 잘 버텼다. 반면에 push를 넣고 training한 컨트롤러 실험의 경우, all crouch motions의 성공률이 꽤 높았다. Crouch 30도가 62.60\%로 가장 높았다.
% 두 경우 모두, crouch 30이 normal gait보다 더 robust한 것을 보였다. 
% \color{red}
% without push controller 중에 each crouch의 성공률을 살펴보면, crouch 정도가 증가할수록 성공률이 증가하였다.
% 단순하게 com이 낮아져서 안정적인 것인지? 아니면 crouch 정도가 증가할 수록 안정적인 foot placement를 할 가능성이 높아지는 것인지.

% detour distance르 살펴보면 오히려 each crouch no push로 실험한 것이 detour distance가 제일 적었다. 성공한 경우들은 normal한 걸음걸이에서 적은 힘으로 밀려서 성공할 수 밖에 없는 모션이었던 것이었다. 의미가 없는 데이터라는 거지 결국....??????  
% \color{black}

% \color{red}
% push training 모션을 밀었을 때와 no push training 모션을 밀었을 때의 반응이 어떻게 다른지! 
% push direction 왼쪽에서만 training 때와 양쪽에서 밀어서 training했을 때 모션이 어떻게 달라지는지!
% 왼쪽, 오른쪽 랜덤으로 밀어서 트레이닝 했을 경우 왼쪽에서만 밀어서 트레이닝했을 때보다 성공률이 더 낮았다 (35.62\% < 54.41\%). 
% \color{black}

% 일단 지금까지의 실험 결과는! 
% 학습 시에 Push 하지 않은 컨트롤러로 시뮬레이션해보니, joint torque model의 경우, 0.2초 동안 190N (mean value에 해당)를 거의 못 버텼다. 작은 힘에 대해서만 견뎠다. 
% push가 training 중간에 들어가지 않으면 cannot withstand large amount of perturbation. 
% 여기서도 normal walking 보다 20, 30도에서 더 잘 버티는 경향성이 나타난다.

% \paragraph{Finding optimal parameter set.}
% DRL을 사용해서 제일 안정적인 crouch angle 및 parameter set을 찾을 수 있지 않을까?
% gradient descent.

% \paragraph{push Mocap mimicking versus normal walking mocap + push simulation training }

% Is there any difference when using push-recovery mocap data as a reference motion and when using the normal walking mocap data with virtual push?
% 기대하기로는 사람을 미는 모습을 모션 캡쳐한 데이터로 컨트롤러를 학습했을 때는 미는 힘에 반응하는 자세 같은 게 엄청 자연스럽게 (팔 모양 같은 거라던가) 나올 것 같다. 그러나 노멀 워킹을 따라가라고 학습하고 시뮬레이션 상에서 외부힘을 가하는 식으로 컨트롤러를 트레이닝했을 때는 아무래도 레퍼런스 모션이 묶여있기 때문에 좀 자연스럽지 않게 나오지 않을까...?  


% \begin{table}
% \caption{Experiment success rate (\%) comparing two control policies with/without external perturbation during training.}
% \begin{tabular}{lccc}
% \toprule
%                         &       DRL-A*  &       DRL-A     \\ \midrule
% Normal                  &      64.04     &                    \\
% Crouch $20\,^{\circ}$   &      72.37     &                   \\ 
% Crouch $30\,^{\circ}$   &      78.61     &                   \\ 
% Crouch $60\,^{\circ}$   &      64.92     &                   \\ 
% \bottomrule
% \end{tabular}
% \bigskip\centering
% \label{tab:Push_success_rate}
% \end{table}



% \paragraph{parameter sampling.}

% % To train a control policy that is robust with various step length and walking speed, we feed the edited motion kinematically to the network to mimic that motion which is parameterized sampled at the normal distribution of each variable. In this case, sampling method can affect the performance of the controller trained with DRL.
% % uniform sampling은 모든 동작 파라미터에 대해서 균등하게 학습하는 방법이고, adaptive는 잘 안 되는 파라미터에 대해서 더 학습하겠다는 건데, 사람이 보통 어떤 동작들을 배울 때는 후자에 가깝게 학습한다.
% % Another factor is that the sampling method can affect the controller trained with DRL.
% % normal distribution을 사용하면 평균 중심에 있는 노말한 모션들이 뽑힐 가능성이 많은데 그렇다면 평균에서 멀리 있는 abnormal 모션들은 많이 안 뽑히기 때문에 학습이 안 될 가능성이 많다. 
% % Uniform sampling을 사용하면 파라미터가 고르게 뽑힌다고 생각할 수 있지만, 성공한 tuple들 위주로 학습이 치우치게 되어 결국에는 평균에서 벗어난 파라미터들로 이루어진 모션은 학습이 잘 안 될 것이다.
% % Recently, Won et al \cite{Won:2019} used adaptive sampling using marginal value function for training the network which is robust to the character's morphology.
% % 우리는 학습할 모션 에디팅에 이 방법을 적용해보기로 했다. adaptive sampling을 쓸 경우에는, 살아남기 힘든 파라미터들에게 학습 기회를 많이 부여하기 때문에 골고루 학습이 잘 될 가능성이 많다.   
% % uniform으로 학습한 것은 모두에게 동일한 기회를 주어 학습한 것이라, 시뮬레이션 실험의 결과가 imitation learning에 있어서 parameter에 따라 만들어지는 보행 모션 각각의 "난이도"를 그대로 의미한다고 볼 수 있는 것 같고,
% % adaptive로 학습한 것은 어려운 동작은 더 많이 기회를 주어서, 어찌 보면 사람과는 좀 다를 수 있는 방식으로 학습하는 것일 수도 있다.

% We use two kinds of sampling methods when training parameterized control policies: one is brute-force sampling, and the other is adaptive sampling, and compare the experimental results of the two.
% As expected, DRL-AD showes more robust results than DRL-BF on push-recovery experiments. The success rates of the adaptive sampling are higher than those of brute-force sampling in every level of crouch (Table ~\ref{fig:Sampling_success_rate}).
% Also, we plot the coverage for two parameters (walking speed and stride length) of each sampling method (Fig. ~\ref{fig:sampling_plot}). Wider range is covered by DRL-AD than DRL-BF. Particularly, adaptive sampling can handle fast gaits with wide stride and slower gaits with short stride.
% Although the two sampling methods have achieved more than 50\% of success rates at all levels of crouches, the most stable crouch level with the highest success rate is different. 
% In the case of DRL-BF, crouch $30\,^{\circ}$ was the highest (72\%), and in the case of DRL-AD, normal walking has the highest rate (80.2\%).
% % 두 샘플링 방법 모두 모든 크라우치 레벨에서 50\%가 넘는 성공률을 보였다. 그러나 가장 성공률이 높은 안정적인 crouch level은 두 경우가 달랐다. uniform의 경우는 crouch 30도가 가장 높았으며, adaptive의 경우는 normal walking이었다. (Fig. ~\ref{fig:sampling_plot}) 을 보면 더 빠르고 보폭이 넓은 걸음에 대해서 adaptive sampling을 사용한 경우 더 안정적으로 나왔다.


% % \begin{table}
% % \caption{Experiment success rate (\%) comparing two control policies with/without adaptive sampling. }
% % \begin{tabular}{lccc}
% % \toprule
% %                         &       DRL-B*          &       DRL-A*          \\ \midrule
% %  Normal                 &       43.32           &       64.04          \\ 
% % Crouch $20\,^{\circ}$   &       63.35           &       72.37            \\ 
% % Crouch $30\,^{\circ}$   &       66.34           &       78.61            \\ 
% % Crouch $60\,^{\circ}$   &       32.33           &       64.92            \\ 
% % \bottomrule
% % \end{tabular}
% % \bigskip\centering
% % \label{fig:Sampling_success_rate}
% % \end{table}


% % Figure
% \begin{figure}
%   \includegraphics[width=\columnwidth]{figures/sampling_comparison_plot.pdf}
%   \caption{Parameter coverages of two sampling methods. Each ellipse represents a 98\% confidence region of a corresponding method.}
%   \label{fig:sampling_plot}
% \end{figure}


% parameter sampling methods(normal, uniform, adaptive) 을 달리해서 training한 결과랑 함께 비교하는 것도 흥미로울 듯.
% 아마도 트레이닝 결과는 Sampling from normal Distribution < sampling from uniform Distribution < adaptive sampling 순일 듯.
% 샘플링 방법에 따라 결과 컨트롤러가 영향을 받는지를 알아보기 위해서 샘플링 방법을 바꿔서 돌려보았다. 
% 고르게 샘플링했을 때 더 넓은 파라미터 변화에도 강건하게 반응하는 모습을 볼 수 있었다...?

% ys: sampling 방식을 달리 해보는 건 의미있는 논의를 할 수 있는 실험인 것 같아.
% normal과 (uniform, adaptive) 비교를 통해 기존에 알려져 있던 대로 sampling을 어떻게 하느냐가 학습 성능에 있어 중요하고, normal distribution은 기존 시뮬레이션 실험 설정과 동일하지만 학습에는 적절치 않다는 얘기를 할 수 있을테고, 하지만 그럼에도 불구하고 어쩌면 이것이 실제 사람이 보행을 학습하는 것과 제일 유사할 수도 있는 것 같고, 그래서 이렇게 학습된 정책으로 시뮬레이션 실험을 해봤을 때 나오는 결과도 의미가 있을 것 같고,
% uniform으로 학습한 것은 모두에게 동일한 기회를 주어 학습한 것이라, 시뮬레이션 실험의 결과가 imitation learning에 있어서 parameter에 따라 만들어지는 보행 모션 각각의 "난이도"를 그대로 의미한다고 볼 수 있는 것 같고,
% adaptive로 학습한 것은 어려운 동작은 더 많이 기회를 주어서, 어찌 보면 사람과는 좀 다를 수 있는 방식으로 학습하는 것일 수도 있고,

% 그래서 이 세 가지 방식으로 학습한 후 각각의 학습된 정책이 시뮬레이션 실험에서
% - 성공 / 실패율이 파라미터에 따라 어떻게 달라지는지 (Table ~\ref{tab:sampling_success})
% - 안정적인 보행을 만드는 파라미터별 경향성이 이 세가지 모두 일치하는지 / 다른지 - 일치해도 의미가 있을 것 같고, 달라도 의미가 있을 것 같아.
% - 각 정잭에 따라 가장 안정적인 crouch angle 및 parameter set이 비슷한지 다른지
% 이런 흥미로운 부분들을 살펴볼 수 있을 것 같아.


